Convex Polytope Modelling for Unsupervised Derivation of Semantic Structure for Data-efficient Natural Language Understanding

Popular approaches for Natural Language Understanding (NLU) usually rely on a huge amount of annotated data or handcrafted rules, which is laborious and not adaptive to domain extension. We recently proposed a Convex-Polytopic-Model-based framework that shows great potential in automatically extracting semantic patterns by exploiting the raw dialog corpus. The extracted semantic patterns can be used to generate semantic frames, which is essential in assisting NLU tasks. This paper further studies the CPM model in depth and visualizes its high interpretability and transparency at various levels. We show that this framework can exploit semantic-frame-related features in the corpus, reveal the underlying semantic structure of the utterances, and boost the performance of the state-of-the-art NLU model with minimal supervision. We conduct our experiments on the ATIS (Air Travel Information System) corpus.

==> Definitions/journalnames.tex <==
\DeclareOption{acoustics}{	\gdef\@journal{acoustics}	\gdef\@journalshort{Acoustics}	\gdef\@journalfull{Acoustics}	\gdef\@doiabbr{acoustics}	\gdef\@ISSN{2624-599X}	}
\DeclareOption{actuators}{	\gdef\@journal{actuators}	\gdef\@journalshort{Actuators}	\gdef\@journalfull{Actuators}	\gdef\@doiabbr{act}	\gdef\@ISSN{2076-0825}	}
\DeclareOption{addictions}{	\gdef\@journal{addictions}	\gdef\@journalshort{Addictions}	\gdef\@journalfull{Addictions}	\gdef\@doiabbr{}	\gdef\@ISSN{0006-0006}	}
\DeclareOption{admsci}{	\gdef\@journal{admsci}	\gdef\@journalshort{Adm. Sci.}	\gdef\@journalfull{Administrative Sciences}	\gdef\@doiabbr{admsci}	\gdef\@ISSN{2076-3387}	}
\DeclareOption{aerospace}{	\gdef\@journal{aerospace}	\gdef\@journalshort{Aerospace}	\gdef\@journalfull{Aerospace}	\gdef\@doiabbr{aerospace}	\gdef\@ISSN{2226-4310}	}
\DeclareOption{agriculture}{	\gdef\@journal{agriculture}	\gdef\@journalshort{Agriculture}	\gdef\@journalfull{Agriculture}	\gdef\@doiabbr{agriculture}	\gdef\@ISSN{2077-0472}	}
\DeclareOption{agriengineering}{	\gdef\@journal{agriengineering}	\gdef\@journalshort{AgriEngineering}	\gdef\@journalfull{AgriEngineering}	\gdef\@doiabbr{agriengineering}	\gdef\@ISSN{2624-7402}	}
\DeclareOption{agronomy}{	\gdef\@journal{agronomy}	\gdef\@journalshort{Agronomy}	\gdef\@journalfull{Agronomy}	\gdef\@doiabbr{agronomy}	\gdef\@ISSN{2073-4395}	}
\DeclareOption{algorithms}{	\gdef\@journal{algorithms}	\gdef\@journalshort{Algorithms}	\gdef\@journalfull{Algorithms}	\gdef\@doiabbr{a}	\gdef\@ISSN{1999-4893}	}
\DeclareOption{animals}{	\gdef\@journal{animals}	\gdef\@journalshort{Animals}	\gdef\@journalfull{Animals}	\gdef\@doiabbr{ani}	\gdef\@ISSN{2076-2615}	}
\DeclareOption{antibiotics}{	\gdef\@journal{antibiotics}	\gdef\@journalshort{Antibiotics}	\gdef\@journalfull{Antibiotics}	\gdef\@doiabbr{antibiotics}	\gdef\@ISSN{2079-6382}	}
\DeclareOption{antibodies}{	\gdef\@journal{antibodies}	\gdef\@journalshort{Antibodies}	\gdef\@journalfull{Antibodies}	\gdef\@doiabbr{antib}	\gdef\@ISSN{2073-4468}	}
\DeclareOption{antioxidants}{	\gdef\@journal{antioxidants}	\gdef\@journalshort{Antioxidants}	\gdef\@journalfull{Antioxidants}	\gdef\@doiabbr{antiox}	\gdef\@ISSN{2076-3921}	}
\DeclareOption{applsci}{	\gdef\@journal{applsci}	\gdef\@journalshort{Appl. Sci.}	\gdef\@journalfull{Applied Sciences}	\gdef\@doiabbr{app}	\gdef\@ISSN{2076-3417}	}
\DeclareOption{arts}{	\gdef\@journal{arts}	\gdef\@journalshort{Arts}	\gdef\@journalfull{Arts}	\gdef\@doiabbr{arts}	\gdef\@ISSN{2076-0752}	}
\DeclareOption{asc}{	\gdef\@journal{asc}	\gdef\@journalshort{Autom. Syst. Control}	\gdef\@journalfull{Automatic Systems and Control}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{asi}{	\gdef\@journal{asi}	\gdef\@journalshort{Appl. Syst. Innov.}	\gdef\@journalfull{Applied System Innovation}	\gdef\@doiabbr{asi}	\gdef\@ISSN{2571-5577}	}
\DeclareOption{atmosphere}{	\gdef\@journal{atmosphere}	\gdef\@journalshort{Atmosphere}	\gdef\@journalfull{Atmosphere}	\gdef\@doiabbr{atmos}	\gdef\@ISSN{2073-4433}	}
\DeclareOption{atoms}{	\gdef\@journal{atoms}	\gdef\@journalshort{Atoms}	\gdef\@journalfull{Atoms}	\gdef\@doiabbr{atoms}	\gdef\@ISSN{2218-2004}	}
\DeclareOption{axioms}{	\gdef\@journal{axioms}	\gdef\@journalshort{Axioms}	\gdef\@journalfull{Axioms}	\gdef\@doiabbr{axioms}	\gdef\@ISSN{2075-1680}	}
\DeclareOption{batteries}{	\gdef\@journal{batteries}	\gdef\@journalshort{Batteries}	\gdef\@journalfull{Batteries}	\gdef\@doiabbr{batteries}	\gdef\@ISSN{2313-0105}	}
\DeclareOption{bdcc}{	\gdef\@journal{bdcc}	\gdef\@journalshort{Big Data Cogn. Comput.}	\gdef\@journalfull{Big Data and Cognitive Computing}	\gdef\@doiabbr{bdcc}	\gdef\@ISSN{2504-2289}	}
\DeclareOption{behavsci}{ 	\gdef\@journal{behavsci} 	\gdef\@journalshort{Behav. Sci.}	\gdef\@journalfull{Behavioral Sciences}	\gdef\@doiabbr{bs}	\gdef\@ISSN{2076-328X}	}
\DeclareOption{beverages}{	\gdef\@journal{beverages}	\gdef\@journalshort{Beverages}	\gdef\@journalfull{Beverages}	\gdef\@doiabbr{beverages}	\gdef\@ISSN{2306-5710}	}
\DeclareOption{bioengineering}{	\gdef\@journal{bioengineering}	\gdef\@journalshort{Bioengineering}	\gdef\@journalfull{Bioengineering}	\gdef\@doiabbr{bioengineering}	\gdef\@ISSN{2306-5354}	}
\DeclareOption{biology}{	\gdef\@journal{biology}	\gdef\@journalshort{Biology}	\gdef\@journalfull{Biology}	\gdef\@doiabbr{biology}	\gdef\@ISSN{2079-7737}	}
\DeclareOption{biomedicines}{	\gdef\@journal{biomedicines}	\gdef\@journalshort{Biomedicines}	\gdef\@journalfull{Biomedicines}	\gdef\@doiabbr{biomedicines}	\gdef\@ISSN{2227-9059}	}
\DeclareOption{biomimetics}{	\gdef\@journal{biomimetics}	\gdef\@journalshort{Biomimetics}	\gdef\@journalfull{Biomimetics}	\gdef\@doiabbr{biomimetics}	\gdef\@ISSN{2313-7673}	}
\DeclareOption{biomolecules}{	\gdef\@journal{biomolecules}	\gdef\@journalshort{Biomolecules}	\gdef\@journalfull{Biomolecules}	\gdef\@doiabbr{biom}	\gdef\@ISSN{2218-273X}	}
\DeclareOption{biosensors}{	\gdef\@journal{biosensors}	\gdef\@journalshort{Biosensors}	\gdef\@journalfull{Biosensors}	\gdef\@doiabbr{bios}	\gdef\@ISSN{2079-6374}	}
\DeclareOption{brainsci}{ 	\gdef\@journal{brainsci} 	\gdef\@journalshort{Brain Sci.}	\gdef\@journalfull{Brain Sciences}	\gdef\@doiabbr{brainsci}	\gdef\@ISSN{2076-3425}	}
\DeclareOption{buildings}{	\gdef\@journal{buildings}	\gdef\@journalshort{Buildings}	\gdef\@journalfull{Buildings}	\gdef\@doiabbr{buildings}	\gdef\@ISSN{2075-5309}	}
\DeclareOption{cancers}{	\gdef\@journal{cancers}	\gdef\@journalshort{Cancers}	\gdef\@journalfull{Cancers}	\gdef\@doiabbr{cancers}	\gdef\@ISSN{2072-6694}	}
\DeclareOption{carbon}{ 	\gdef\@journal{carbon} 	\gdef\@journalshort{C}	\gdef\@journalfull{C}	\gdef\@doiabbr{c}	\gdef\@ISSN{2311-5629}	}
\DeclareOption{catalysts}{	\gdef\@journal{catalysts}	\gdef\@journalshort{Catalysts}	\gdef\@journalfull{Catalysts}	\gdef\@doiabbr{catal}	\gdef\@ISSN{2073-4344}	}
\DeclareOption{cells}{	\gdef\@journal{cells}	\gdef\@journalshort{Cells}	\gdef\@journalfull{Cells}	\gdef\@doiabbr{cells}	\gdef\@ISSN{2073-4409}	}
\DeclareOption{ceramics}{	\gdef\@journal{ceramics}	\gdef\@journalshort{Ceramics}	\gdef\@journalfull{Ceramics}	\gdef\@doiabbr{ceramics}	\gdef\@ISSN{2571-6131}	}
\DeclareOption{challenges}{	\gdef\@journal{challenges}	\gdef\@journalshort{Challenges}	\gdef\@journalfull{Challenges}	\gdef\@doiabbr{challe}	\gdef\@ISSN{2078-1547}	}
\DeclareOption{chemengineering}{	\gdef\@journal{chemengineering}	\gdef\@journalshort{ChemEngineering}	\gdef\@journalfull{ChemEngineering}	\gdef\@doiabbr{chemengineering}	\gdef\@ISSN{2305-7084}	}
\DeclareOption{chemistry}{	\gdef\@journal{chemistry}	\gdef\@journalshort{Chemistry}	\gdef\@journalfull{Chemistry}	\gdef\@doiabbr{chemistry}	\gdef\@ISSN{2624-8549}	}
\DeclareOption{chemosensors}{	\gdef\@journal{chemosensors}	\gdef\@journalshort{Chemosensors}	\gdef\@journalfull{Chemosensors}	\gdef\@doiabbr{chemosensors}	\gdef\@ISSN{2227-9040}	}
\DeclareOption{children}{	\gdef\@journal{children}	\gdef\@journalshort{Children}	\gdef\@journalfull{Children}	\gdef\@doiabbr{children}	\gdef\@ISSN{2227-9067}	}
\DeclareOption{cleantechnol}{	\gdef\@journal{cleantechnol}	\gdef\@journalshort{Clean Technol.}	\gdef\@journalfull{Clean Technologies}	\gdef\@doiabbr{cleantechnol}	\gdef\@ISSN{2571-8797}	}
\DeclareOption{climate}{	\gdef\@journal{climate}	\gdef\@journalshort{Climate}	\gdef\@journalfull{Climate}	\gdef\@doiabbr{cli}	\gdef\@ISSN{2225-1154}	}
\DeclareOption{clockssleep}{	\gdef\@journal{clockssleep}	\gdef\@journalshort{Clocks\&Sleep}	\gdef\@journalfull{Clocks \& Sleep}	\gdef\@doiabbr{clockssleep}	\gdef\@ISSN{2624-5175}	}
\DeclareOption{cmd}{	\gdef\@journal{cmd}	\gdef\@journalshort{Corros. Mater. Degrad.}	\gdef\@journalfull{Corrosion and Materials Degradation}	\gdef\@doiabbr{cmd}	\gdef\@ISSN{2624-5558}	}
\DeclareOption{coatings}{	\gdef\@journal{coatings}	\gdef\@journalshort{Coatings}	\gdef\@journalfull{Coatings}	\gdef\@doiabbr{coatings}	\gdef\@ISSN{2079-6412}	}
\DeclareOption{colloids}{	\gdef\@journal{colloids}	\gdef\@journalshort{Colloids Interfaces}	\gdef\@journalfull{Colloids Interfaces}	\gdef\@doiabbr{colloids}	\gdef\@ISSN{2504-5377}	}
\DeclareOption{computation}{	\gdef\@journal{computation}	\gdef\@journalshort{Computation}	\gdef\@journalfull{Computation}	\gdef\@doiabbr{computation}	\gdef\@ISSN{2079-3197}	}
\DeclareOption{computers}{	\gdef\@journal{computers}	\gdef\@journalshort{Computers}	\gdef\@journalfull{Computers}	\gdef\@doiabbr{computers}	\gdef\@ISSN{2073-431X}	}
\DeclareOption{condensedmatter}{	\gdef\@journal{condensedmatter}	\gdef\@journalshort{Condens. Matter}	\gdef\@journalfull{Condensed Matter}	\gdef\@doiabbr{condmat}	\gdef\@ISSN{2410-3896}	}
\DeclareOption{cosmetics}{	\gdef\@journal{cosmetics}	\gdef\@journalshort{Cosmetics}	\gdef\@journalfull{Cosmetics}	\gdef\@doiabbr{cosmetics}	\gdef\@ISSN{2079-9284}	}
\DeclareOption{cryptography}{	\gdef\@journal{cryptography}	\gdef\@journalshort{Cryptography}	\gdef\@journalfull{Cryptography}	\gdef\@doiabbr{cryptography}	\gdef\@ISSN{2410-387X}	}
\DeclareOption{crystals}{	\gdef\@journal{crystals}	\gdef\@journalshort{Crystals}	\gdef\@journalfull{Crystals}	\gdef\@doiabbr{cryst}	\gdef\@ISSN{2073-4352}	}
\DeclareOption{dairy}{	\gdef\@journal{dairy}	\gdef\@journalshort{Dairy}	\gdef\@journalfull{Dairy}	\gdef\@doiabbr{dairy}	\gdef\@ISSN{2624-862X}	}
\DeclareOption{data}{	\gdef\@journal{data}	\gdef\@journalshort{Data}	\gdef\@journalfull{Data}	\gdef\@doiabbr{data}	\gdef\@ISSN{2306-5729}	}
\DeclareOption{dentistry}{	\gdef\@journal{dentistry}	\gdef\@journalshort{Dent. J.}	\gdef\@journalfull{Dentistry Journal}	\gdef\@doiabbr{dj}	\gdef\@ISSN{2304-6767}	}
\DeclareOption{designs}{ 	\gdef\@journal{designs} 	\gdef\@journalshort{Designs}	\gdef\@journalfull{Designs}	\gdef\@doiabbr{designs}	\gdef\@ISSN{2411-9660}	}
\DeclareOption{diagnostics}{	\gdef\@journal{diagnostics}	\gdef\@journalshort{Diagnostics}	\gdef\@journalfull{Diagnostics}	\gdef\@doiabbr{diagnostics}	\gdef\@ISSN{2075-4418}	}
\DeclareOption{diseases}{	\gdef\@journal{diseases}	\gdef\@journalshort{Diseases}	\gdef\@journalfull{Diseases}	\gdef\@doiabbr{diseases}	\gdef\@ISSN{2079-9721}	}
\DeclareOption{diversity}{	\gdef\@journal{diversity}	\gdef\@journalshort{Diversity}	\gdef\@journalfull{Diversity}	\gdef\@doiabbr{d}	\gdef\@ISSN{1424-2818}	}
\DeclareOption{drones}{	\gdef\@journal{drones}	\gdef\@journalshort{Drones}	\gdef\@journalfull{Drones}	\gdef\@doiabbr{drones}	\gdef\@ISSN{2504-446X}	}
\DeclareOption{econometrics}{	\gdef\@journal{econometrics}	\gdef\@journalshort{Econometrics}	\gdef\@journalfull{Econometrics}	\gdef\@doiabbr{econometrics}	\gdef\@ISSN{2225-1146}	}
\DeclareOption{economies}{	\gdef\@journal{economies}	\gdef\@journalshort{Economies}	\gdef\@journalfull{Economies}	\gdef\@doiabbr{economies}	\gdef\@ISSN{2227-7099}	}
\DeclareOption{education}{	\gdef\@journal{education}	\gdef\@journalshort{Educ. Sci.}	\gdef\@journalfull{Education Sciences}	\gdef\@doiabbr{educsci}	\gdef\@ISSN{2227-7102}	}
\DeclareOption{ejihpe}{	\gdef\@journal{ejihpe}	\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}	\gdef\@journalfull{European Journal of Investigation in Health, Psychology and Education}	\gdef\@doiabbr{ejihpe}	\gdef\@ISSN{2254-9625}	}
\DeclareOption{electrochem}{	\gdef\@journal{electrochem}	\gdef\@journalshort{Electrochem}	\gdef\@journalfull{Electrochem}	\gdef\@doiabbr{electrochem}	\gdef\@ISSN{}	}
\DeclareOption{electronics}{	\gdef\@journal{electronics}	\gdef\@journalshort{Electronics}	\gdef\@journalfull{Electronics}	\gdef\@doiabbr{electronics}	\gdef\@ISSN{2079-9292}	}
\DeclareOption{energies}{	\gdef\@journal{energies}	\gdef\@journalshort{Energies}	\gdef\@journalfull{Energies}	\gdef\@doiabbr{en}	\gdef\@ISSN{1996-1073}	}
\DeclareOption{entropy}{	\gdef\@journal{entropy}	\gdef\@journalshort{Entropy}	\gdef\@journalfull{Entropy}	\gdef\@doiabbr{e}	\gdef\@ISSN{1099-4300}	}
\DeclareOption{environments}{	\gdef\@journal{environments}	\gdef\@journalshort{Environments}	\gdef\@journalfull{Environments}	\gdef\@doiabbr{environments}	\gdef\@ISSN{2076-3298}	}
\DeclareOption{epigenomes}{	\gdef\@journal{epigenomes}	\gdef\@journalshort{Epigenomes}	\gdef\@journalfull{Epigenomes}	\gdef\@doiabbr{epigenomes}	\gdef\@ISSN{2075-4655}	}
\DeclareOption{est}{	\gdef\@journal{est}	\gdef\@journalshort{Electrochem. Sci. Technol.}	\gdef\@journalfull{Electrochemical Science and Technology}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{fermentation}{	\gdef\@journal{fermentation}	\gdef\@journalshort{Fermentation}	\gdef\@journalfull{Fermentation}	\gdef\@doiabbr{fermentation}	\gdef\@ISSN{2311-5637}	}
\DeclareOption{fibers}{	\gdef\@journal{fibers}	\gdef\@journalshort{Fibers}	\gdef\@journalfull{Fibers}	\gdef\@doiabbr{fib}	\gdef\@ISSN{2079-6439}	}
\DeclareOption{fire}{	\gdef\@journal{fire}	\gdef\@journalshort{Fire}	\gdef\@journalfull{Fire}	\gdef\@doiabbr{fire}	\gdef\@ISSN{2571-6255}	}
\DeclareOption{fishes}{	\gdef\@journal{fishes}	\gdef\@journalshort{Fishes}	\gdef\@journalfull{Fishes}	\gdef\@doiabbr{fishes}	\gdef\@ISSN{2410-3888}	}
\DeclareOption{fluids}{	\gdef\@journal{fluids}	\gdef\@journalshort{Fluids}	\gdef\@journalfull{Fluids}	\gdef\@doiabbr{fluids}	\gdef\@ISSN{2311-5521}	}
\DeclareOption{foods}{	\gdef\@journal{foods}	\gdef\@journalshort{Foods}	\gdef\@journalfull{Foods}	\gdef\@doiabbr{foods}	\gdef\@ISSN{2304-8158}	}
\DeclareOption{forecasting}{	\gdef\@journal{forecasting}	\gdef\@journalshort{Forecasting}	\gdef\@journalfull{Forecasting}	\gdef\@doiabbr{forecast}	\gdef\@ISSN{2571-9394}	}
\DeclareOption{forests}{	\gdef\@journal{forests}	\gdef\@journalshort{Forests}	\gdef\@journalfull{Forests}	\gdef\@doiabbr{f}	\gdef\@ISSN{1999-4907}	}
\DeclareOption{fractalfract}{	\gdef\@journal{fractalfract}	\gdef\@journalshort{Fractal Fract.}	\gdef\@journalfull{Fractal and Fractional}	\gdef\@doiabbr{fractalfract}	\gdef\@ISSN{2504-3110}	}
\DeclareOption{futureinternet}{	\gdef\@journal{futureinternet}	\gdef\@journalshort{Future Internet}	\gdef\@journalfull{Future Internet}	\gdef\@doiabbr{fi}	\gdef\@ISSN{1999-5903}	}
\DeclareOption{futurephys}{	\gdef\@journal{futurephys}	\gdef\@journalshort{Future Phys.}	\gdef\@journalfull{Future Physics}	\gdef\@doiabbr{futurephys}	\gdef\@ISSN{2624-6503}	}
\DeclareOption{galaxies}{	\gdef\@journal{galaxies}	\gdef\@journalshort{Galaxies}	\gdef\@journalfull{Galaxies}	\gdef\@doiabbr{galaxies}	\gdef\@ISSN{2075-4434}	}
\DeclareOption{games}{	\gdef\@journal{games}	\gdef\@journalshort{Games}	\gdef\@journalfull{Games}	\gdef\@doiabbr{g}	\gdef\@ISSN{2073-4336}	}
\DeclareOption{gastrointestdisord}{	\gdef\@journal{gastrointestdisord}	\gdef\@journalshort{Gastrointest. Disord.}	\gdef\@journalfull{Gastrointestinal Disorders}	\gdef\@doiabbr{gidisord}	\gdef\@ISSN{2624-5647}	}
\DeclareOption{gels}{	\gdef\@journal{gels}	\gdef\@journalshort{Gels}	\gdef\@journalfull{Gels}	\gdef\@doiabbr{gels}	\gdef\@ISSN{2310-2861}	}
\DeclareOption{genealogy}{	\gdef\@journal{genealogy}	\gdef\@journalshort{Genealogy}	\gdef\@journalfull{Genealogy}	\gdef\@doiabbr{genealogy}	\gdef\@ISSN{2313-5778}	}
\DeclareOption{genes}{	\gdef\@journal{genes}	\gdef\@journalshort{Genes}	\gdef\@journalfull{Genes}	\gdef\@doiabbr{genes}	\gdef\@ISSN{2073-4425}	}
\DeclareOption{geohazards}{	\gdef\@journal{geohazards}	\gdef\@journalshort{GeoHazards}	\gdef\@journalfull{GeoHazards}	\gdef\@doiabbr{geohazards}	\gdef\@ISSN{2624-795X}	}
\DeclareOption{geosciences}{	\gdef\@journal{geosciences}	\gdef\@journalshort{Geosciences}	\gdef\@journalfull{Geosciences}	\gdef\@doiabbr{geosciences}	\gdef\@ISSN{2076-3263}	}
\DeclareOption{geriatrics}{	\gdef\@journal{geriatrics}	\gdef\@journalshort{Geriatrics}	\gdef\@journalfull{Geriatrics}	\gdef\@doiabbr{geriatrics}	\gdef\@ISSN{2308-3417}	}
\DeclareOption{hazardousmatters}{	\gdef\@journal{hazardousmatters}	\gdef\@journalshort{Hazard. Matters}	\gdef\@journalfull{Hazardous Matters}	\gdef\@doiabbr{}	\gdef\@ISSN{0014-0014}	}
\DeclareOption{healthcare}{	\gdef\@journal{healthcare}	\gdef\@journalshort{Healthcare}	\gdef\@journalfull{Healthcare}	\gdef\@doiabbr{healthcare}	\gdef\@ISSN{2227-9032}	}
\DeclareOption{heritage}{	\gdef\@journal{heritage}	\gdef\@journalshort{Heritage}	\gdef\@journalfull{Heritage}	\gdef\@doiabbr{heritage}	\gdef\@ISSN{2571-9408}	}
\DeclareOption{highthroughput}{	\gdef\@journal{highthroughput}	\gdef\@journalshort{High-Throughput}	\gdef\@journalfull{High-Throughput}	\gdef\@doiabbr{ht}	\gdef\@ISSN{2571-5135}	}
\DeclareOption{horticulturae}{	\gdef\@journal{horticulturae}	\gdef\@journalshort{Horticulturae}	\gdef\@journalfull{Horticulturae}	\gdef\@doiabbr{horticulturae}	\gdef\@ISSN{2311-7524}	}
\DeclareOption{humanities}{	\gdef\@journal{humanities}	\gdef\@journalshort{Humanities}	\gdef\@journalfull{Humanities}	\gdef\@doiabbr{h}	\gdef\@ISSN{2076-0787}	}
\DeclareOption{hydrology}{	\gdef\@journal{hydrology}	\gdef\@journalshort{Hydrology}	\gdef\@journalfull{Hydrology}	\gdef\@doiabbr{hydrology}	\gdef\@ISSN{2306-5338}	}
\DeclareOption{ijerph}{	\gdef\@journal{ijerph}	\gdef\@journalshort{Int. J. Environ. Res. Public Health}	\gdef\@journalfull{International Journal of Environmental Research and Public Health}	\gdef\@doiabbr{ijerph}	\gdef\@ISSN{1660-4601}	}
\DeclareOption{ijfs}{	\gdef\@journal{ijfs}	\gdef\@journalshort{Int. J. Financial Stud.}	\gdef\@journalfull{International Journal of Financial Studies}	\gdef\@doiabbr{ijfs}	\gdef\@ISSN{2227-7072}	}
\DeclareOption{ijgi}{	\gdef\@journal{ijgi}	\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}	\gdef\@journalfull{ISPRS International Journal of Geo-Information}	\gdef\@doiabbr{ijgi}	\gdef\@ISSN{2220-9964}	}
\DeclareOption{ijms}{	\gdef\@journal{ijms}	\gdef\@journalshort{Int. J. Mol. Sci.}	\gdef\@journalfull{International Journal of Molecular Sciences}	\gdef\@doiabbr{ijms}	\gdef\@ISSN{1422-0067}	}
\DeclareOption{ijtpp}{	\gdef\@journal{ijtpp}	\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}	\gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}	\gdef\@doiabbr{ijtpp}	\gdef\@ISSN{2504-186X}	}
\DeclareOption{informatics}{	\gdef\@journal{informatics}	\gdef\@journalshort{Informatics}	\gdef\@journalfull{Informatics}	\gdef\@doiabbr{informatics}	\gdef\@ISSN{2227-9709}	}
\DeclareOption{information}{	\gdef\@journal{information}	\gdef\@journalshort{Information}	\gdef\@journalfull{Information}	\gdef\@doiabbr{info}	\gdef\@ISSN{2078-2489}	}
\DeclareOption{infrastructures}{	\gdef\@journal{infrastructures}	\gdef\@journalshort{Infrastructures}	\gdef\@journalfull{Infrastructures}	\gdef\@doiabbr{infrastructures}	\gdef\@ISSN{2412-3811}	}
\DeclareOption{inorganics}{	\gdef\@journal{inorganics}	\gdef\@journalshort{Inorganics}	\gdef\@journalfull{Inorganics}	\gdef\@doiabbr{inorganics}	\gdef\@ISSN{2304-6740}	}
\DeclareOption{insects}{	\gdef\@journal{insects}	\gdef\@journalshort{Insects}	\gdef\@journalfull{Insects}	\gdef\@doiabbr{insects}	\gdef\@ISSN{2075-4450}	}
\DeclareOption{instruments}{	\gdef\@journal{instruments}	\gdef\@journalshort{Instruments}	\gdef\@journalfull{Instruments}	\gdef\@doiabbr{instruments}	\gdef\@ISSN{2410-390X}	}
\DeclareOption{inventions}{	\gdef\@journal{inventions}	\gdef\@journalshort{Inventions}	\gdef\@journalfull{Inventions}	\gdef\@doiabbr{inventions}	\gdef\@ISSN{2411-5134}	}
\DeclareOption{iot}{	\gdef\@journal{iot}	\gdef\@journalshort{IoT}	\gdef\@journalfull{IoT}	\gdef\@doiabbr{iot}	\gdef\@ISSN{2624-831X}	}
\DeclareOption{j}{	\gdef\@journal{j}	\gdef\@journalshort{J}	\gdef\@journalfull{J}	\gdef\@doiabbr{j}	\gdef\@ISSN{2571-8800}	}
\DeclareOption{jcdd}{	\gdef\@journal{jcdd}	\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}	\gdef\@journalfull{Journal of Cardiovascular Development and Disease}	\gdef\@doiabbr{jcdd}	\gdef\@ISSN{2308-3425}	}
\DeclareOption{jcm}{	\gdef\@journal{jcm}	\gdef\@journalshort{J. Clin. Med.}	\gdef\@journalfull{Journal of Clinical Medicine}	\gdef\@doiabbr{jcm}	\gdef\@ISSN{2077-0383}	}
\DeclareOption{jcp}{	\gdef\@journal{jcp}	\gdef\@journalshort{J. Cybersecur. Priv.}	\gdef\@journalfull{Journal of Cybersecurity and Privacy}	\gdef\@doiabbr{jcp}	\gdef\@ISSN{2624-800X}	}
\DeclareOption{jcs}{	\gdef\@journal{jcs}	\gdef\@journalshort{J. Compos. Sci.}	\gdef\@journalfull{Journal of Composites Science}	\gdef\@doiabbr{jcs}	\gdef\@ISSN{2504-477X}	}
\DeclareOption{jdb}{	\gdef\@journal{jdb}	\gdef\@journalshort{J. Dev. Biol.}	\gdef\@journalfull{Journal of Developmental Biology}	\gdef\@doiabbr{jdb}	\gdef\@ISSN{2221-3759}	}
\DeclareOption{jfb}{	\gdef\@journal{jfb}	\gdef\@journalshort{J. Funct. Biomater.}   	\gdef\@journalfull{Journal of Functional Biomaterials}   	\gdef\@doiabbr{jfb}	\gdef\@ISSN{2079-4983}	}
\DeclareOption{jfmk}{	\gdef\@journal{jfmk}	\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}   	\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}   	\gdef\@doiabbr{jfmk}	\gdef\@ISSN{2411-5142}	}
\DeclareOption{jimaging}{	\gdef\@journal{jimaging}	\gdef\@journalshort{J. Imaging}	\gdef\@journalfull{Journal of Imaging}	\gdef\@doiabbr{jimaging}	\gdef\@ISSN{2313-433X}	}
\DeclareOption{jintelligence}{	\gdef\@journal{jintelligence}	\gdef\@journalshort{J. Intell.}	\gdef\@journalfull{Journal of Intelligence}	\gdef\@doiabbr{jintelligence}	\gdef\@ISSN{2079-3200}	}
\DeclareOption{jlpea}{	\gdef\@journal{jlpea}	\gdef\@journalshort{J. Low Power Electron. Appl.}	\gdef\@journalfull{Journal of Low Power Electronics and Applications}	\gdef\@doiabbr{jlpea}	\gdef\@ISSN{2079-9268}	}
\DeclareOption{jmmp}{	\gdef\@journal{jmmp}	\gdef\@journalshort{J. Manuf. Mater. Process.}	\gdef\@journalfull{Journal of Manufacturing and Materials Processing}	\gdef\@doiabbr{jmmp}	\gdef\@ISSN{2504-4494}	}
\DeclareOption{jmse}{	\gdef\@journal{jmse}	\gdef\@journalshort{J. Mar. Sci. Eng.}	\gdef\@journalfull{Journal of Marine Science and Engineering}	\gdef\@doiabbr{jmse}	\gdef\@ISSN{2077-1312}	}
\DeclareOption{jnt}{	\gdef\@journal{jnt}	\gdef\@journalshort{J. Nanotheranostics}	\gdef\@journalfull{Journal of Nanotheranostics}	\gdef\@doiabbr{jnt}	\gdef\@ISSN{2624-845X}	}
\DeclareOption{jof}{	\gdef\@journal{jof}	\gdef\@journalshort{J. Fungi}	\gdef\@journalfull{Journal of Fungi}	\gdef\@doiabbr{jof}	\gdef\@ISSN{2309-608X}	}
\DeclareOption{joitmc}{	\gdef\@journal{joitmc}	\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}	\gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}	\gdef\@doiabbr{joitmc}	\gdef\@ISSN{2199-8531}	}
\DeclareOption{jpm}{	\gdef\@journal{jpm}	\gdef\@journalshort{J. Pers. Med.}	\gdef\@journalfull{Journal of Personalized Medicine}	\gdef\@doiabbr{jpm}	\gdef\@ISSN{2075-4426}	}
\DeclareOption{jrfm}{	\gdef\@journal{jrfm}	\gdef\@journalshort{J. Risk Financial Manag.}	\gdef\@journalfull{Journal of Risk and Financial Management}	\gdef\@doiabbr{jrfm}	\gdef\@ISSN{1911-8074}	}
\DeclareOption{jsan}{	\gdef\@journal{jsan}	\gdef\@journalshort{J. Sens. Actuator Netw.}	\gdef\@journalfull{Journal of Sensor and Actuator Networks}	\gdef\@doiabbr{jsan}	\gdef\@ISSN{2224-2708}	}
\DeclareOption{land}{	\gdef\@journal{land}	\gdef\@journalshort{Land}	\gdef\@journalfull{Land}	\gdef\@doiabbr{land}	\gdef\@ISSN{2073-445X}	}
\DeclareOption{languages}{	\gdef\@journal{languages}	\gdef\@journalshort{Languages}	\gdef\@journalfull{Languages}	\gdef\@doiabbr{languages}	\gdef\@ISSN{2226-471X}	}
\DeclareOption{laws}{	\gdef\@journal{laws}	\gdef\@journalshort{Laws}	\gdef\@journalfull{Laws}	\gdef\@doiabbr{laws}	\gdef\@ISSN{2075-471X}	}
\DeclareOption{life}{	\gdef\@journal{life}	\gdef\@journalshort{Life}	\gdef\@journalfull{Life}	\gdef\@doiabbr{life}	\gdef\@ISSN{2075-1729}	}
\DeclareOption{literature}{	\gdef\@journal{literature}	\gdef\@journalshort{Literature}	\gdef\@journalfull{Literature}	\gdef\@doiabbr{}	\gdef\@ISSN{2410-9789}	}
\DeclareOption{logistics}{	\gdef\@journal{logistics}	\gdef\@journalshort{Logistics}	\gdef\@journalfull{Logistics}	\gdef\@doiabbr{logistics}	\gdef\@ISSN{2305-6290}	}
\DeclareOption{lubricants}{	\gdef\@journal{lubricants}	\gdef\@journalshort{Lubricants}	\gdef\@journalfull{Lubricants}	\gdef\@doiabbr{lubricants}	\gdef\@ISSN{2075-4442}	}
\DeclareOption{machines}{	\gdef\@journal{machines}	\gdef\@journalshort{Machines}	\gdef\@journalfull{Machines}	\gdef\@doiabbr{machines}	\gdef\@ISSN{2075-1702}	}
\DeclareOption{magnetochemistry}{	\gdef\@journal{magnetochemistry}	\gdef\@journalshort{Magnetochemistry}	\gdef\@journalfull{Magnetochemistry}	\gdef\@doiabbr{magnetochemistry}	\gdef\@ISSN{2312-7481}	}
\DeclareOption{make}{	\gdef\@journal{make}	\gdef\@journalshort{Mach. Learn. Knowl. Extr.}	\gdef\@journalfull{Machine Learning and Knowledge Extraction}	\gdef\@doiabbr{make}	\gdef\@ISSN{2504-4990}	}
\DeclareOption{marinedrugs}{	\gdef\@journal{marinedrugs}	\gdef\@journalshort{Mar. Drugs}	\gdef\@journalfull{Marine Drugs}	\gdef\@doiabbr{md}	\gdef\@ISSN{1660-3397}	}
\DeclareOption{materials}{	\gdef\@journal{materials}	\gdef\@journalshort{Materials}	\gdef\@journalfull{Materials}	\gdef\@doiabbr{ma}	\gdef\@ISSN{1996-1944}	}
\DeclareOption{mathematics}{	\gdef\@journal{mathematics}	\gdef\@journalshort{Mathematics}	\gdef\@journalfull{Mathematics}	\gdef\@doiabbr{math}	\gdef\@ISSN{2227-7390}	}
\DeclareOption{mca}{	\gdef\@journal{mca}	\gdef\@journalshort{Math. Comput. Appl.}	\gdef\@journalfull{Mathematical and Computational Applications}	\gdef\@doiabbr{mca}	\gdef\@ISSN{2297-8747}	}
\DeclareOption{medicina}{	\gdef\@journal{medicina}	\gdef\@journalshort{Medicina}	\gdef\@journalfull{Medicina}	\gdef\@doiabbr{medicina}	\gdef\@ISSN{1010-660X}	}
\DeclareOption{medicines}{	\gdef\@journal{medicines}	\gdef\@journalshort{Medicines}	\gdef\@journalfull{Medicines}	\gdef\@doiabbr{medicines}	\gdef\@ISSN{2305-6320}	}
\DeclareOption{medsci}{	\gdef\@journal{medsci}	\gdef\@journalshort{Med. Sci.}	\gdef\@journalfull{Medical Sciences}	\gdef\@doiabbr{medsci}	\gdef\@ISSN{2076-3271}	}
\DeclareOption{membranes}{	\gdef\@journal{membranes}	\gdef\@journalshort{Membranes}	\gdef\@journalfull{Membranes}	\gdef\@doiabbr{membranes}	\gdef\@ISSN{2077-0375}	}
\DeclareOption{metabolites}{	\gdef\@journal{metabolites}	\gdef\@journalshort{Metabolites}	\gdef\@journalfull{Metabolites}	\gdef\@doiabbr{metabo}	\gdef\@ISSN{2218-1989}	}
\DeclareOption{metals}{	\gdef\@journal{metals}	\gdef\@journalshort{Metals}	\gdef\@journalfull{Metals}	\gdef\@doiabbr{met}	\gdef\@ISSN{2075-4701}	}
\DeclareOption{microarrays}{	\gdef\@journal{microarrays}	\gdef\@journalshort{Microarrays}	\gdef\@journalfull{Microarrays}	\gdef\@doiabbr{}	\gdef\@ISSN{2076-3905}	}
\DeclareOption{micromachines}{	\gdef\@journal{micromachines}	\gdef\@journalshort{Micromachines}	\gdef\@journalfull{Micromachines}	\gdef\@doiabbr{mi}	\gdef\@ISSN{2072-666X}	}
\DeclareOption{microorganisms}{	\gdef\@journal{microorganisms}	\gdef\@journalshort{Microorganisms}	\gdef\@journalfull{Microorganisms}	\gdef\@doiabbr{microorganisms}	\gdef\@ISSN{2076-2607}	}
\DeclareOption{minerals}{	\gdef\@journal{minerals}	\gdef\@journalshort{Minerals}	\gdef\@journalfull{Minerals}	\gdef\@doiabbr{min}	\gdef\@ISSN{2075-163X}	}
\DeclareOption{modelling}{	\gdef\@journal{modelling}	\gdef\@journalshort{Modelling}	\gdef\@journalfull{Modelling}	\gdef\@doiabbr{}	\gdef\@ISSN{0012-0012}	}
\DeclareOption{molbank}{	\gdef\@journal{molbank}	\gdef\@journalshort{Molbank}	\gdef\@journalfull{Molbank}	\gdef\@doiabbr{M}	\gdef\@ISSN{1422-8599}	}
\DeclareOption{molecules}{	\gdef\@journal{molecules}	\gdef\@journalshort{Molecules}	\gdef\@journalfull{Molecules}	\gdef\@doiabbr{molecules}	\gdef\@ISSN{1420-3049}	}
\DeclareOption{mps}{	\gdef\@journal{mps}	\gdef\@journalshort{Methods Protoc.}	\gdef\@journalfull{Methods and Protocols}	\gdef\@doiabbr{mps}	\gdef\@ISSN{2409-9279}	}
\DeclareOption{mti}{	\gdef\@journal{mti}	\gdef\@journalshort{Multimodal Technol. Interact.}	\gdef\@journalfull{Multimodal Technologies and Interaction}	\gdef\@doiabbr{mti}	\gdef\@ISSN{2414-4088}	}
\DeclareOption{nanomaterials}{	\gdef\@journal{nanomaterials}	\gdef\@journalshort{Nanomaterials}	\gdef\@journalfull{Nanomaterials}	\gdef\@doiabbr{nano}	\gdef\@ISSN{2079-4991}	}
\DeclareOption{ncrna}{	\gdef\@journal{ncrna}	\gdef\@journalshort{Non-coding RNA}	\gdef\@journalfull{Non-coding RNA}	\gdef\@doiabbr{ncrna}	\gdef\@ISSN{2311-553X}	}
\DeclareOption{ijns}{	\gdef\@journal{ijns}	\gdef\@journalshort{Int. J. Neonatal Screen.}	\gdef\@journalfull{International Journal of Neonatal Screening}	\gdef\@doiabbr{ijns}	\gdef\@ISSN{2409-515X}	}
\DeclareOption{neuroglia}{	\gdef\@journal{neuroglia}	\gdef\@journalshort{Neuroglia}	\gdef\@journalfull{Neuroglia}	\gdef\@doiabbr{neuroglia}	\gdef\@ISSN{2571-6980}	}
\DeclareOption{nitrogen}{	\gdef\@journal{nitrogen}	\gdef\@journalshort{Nitrogen}	\gdef\@journalfull{Nitrogen}	\gdef\@doiabbr{nitrogen}	\gdef\@ISSN{2504-3129}	}
\DeclareOption{notspecified}{	\gdef\@journal{notspecified}	\gdef\@journalshort{Journal Not Specified}	\gdef\@journalfull{Journal Not Specified}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{nutrients}{	\gdef\@journal{nutrients}	\gdef\@journalshort{Nutrients}	\gdef\@journalfull{Nutrients}	\gdef\@doiabbr{nu}	\gdef\@ISSN{2072-6643}	}
\DeclareOption{ohbm}{	\gdef\@journal{ohbm}	\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}	\gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}	\gdef\@doiabbr{ohbm}	\gdef\@ISSN{2504-463X}	}
\DeclareOption{optics}{	\gdef\@journal{optics}	\gdef\@journalshort{Optics}	\gdef\@journalfull{Optics}	\gdef\@doiabbr{opt}	\gdef\@ISSN{}	}
\DeclareOption{particles}{	\gdef\@journal{particles}	\gdef\@journalshort{Particles}	\gdef\@journalfull{Particles}	\gdef\@doiabbr{particles}	\gdef\@ISSN{2571-712X}	}
\DeclareOption{pathogens}{	\gdef\@journal{pathogens}	\gdef\@journalshort{Pathogens}	\gdef\@journalfull{Pathogens}	\gdef\@doiabbr{pathogens}	\gdef\@ISSN{2076-0817}	}
\DeclareOption{pharmaceuticals}{	\gdef\@journal{pharmaceuticals}	\gdef\@journalshort{Pharmaceuticals}	\gdef\@journalfull{Pharmaceuticals}	\gdef\@doiabbr{ph}	\gdef\@ISSN{1424-8247}	}
\DeclareOption{pharmaceutics}{	\gdef\@journal{pharmaceutics}	\gdef\@journalshort{Pharmaceutics}	\gdef\@journalfull{Pharmaceutics}	\gdef\@doiabbr{pharmaceutics}	\gdef\@ISSN{1999-4923}	}
\DeclareOption{pharmacy}{	\gdef\@journal{pharmacy}	\gdef\@journalshort{Pharmacy}	\gdef\@journalfull{Pharmacy}	\gdef\@doiabbr{pharmacy}	\gdef\@ISSN{2226-4787}	}
\DeclareOption{philosophies}{	\gdef\@journal{philosophies}	\gdef\@journalshort{Philosophies}	\gdef\@journalfull{Philosophies}	\gdef\@doiabbr{philosophies}	\gdef\@ISSN{2409-9287}	}
\DeclareOption{photonics}{	\gdef\@journal{photonics}	\gdef\@journalshort{Photonics}	\gdef\@journalfull{Photonics}	\gdef\@doiabbr{photonics}	\gdef\@ISSN{2304-6732}	}
\DeclareOption{physics}{	\gdef\@journal{physics}	\gdef\@journalshort{Physics}	\gdef\@journalfull{Physics}	\gdef\@doiabbr{physics}	\gdef\@ISSN{2624-8174}	}
\DeclareOption{plants}{	\gdef\@journal{plants}	\gdef\@journalshort{Plants}	\gdef\@journalfull{Plants}	\gdef\@doiabbr{plants}	\gdef\@ISSN{2223-7747}	}
\DeclareOption{plasma}{	\gdef\@journal{plasma}	\gdef\@journalshort{Plasma}	\gdef\@journalfull{Plasma}	\gdef\@doiabbr{plasma}	\gdef\@ISSN{2571-6182}	}
\DeclareOption{polymers}{	\gdef\@journal{polymers}	\gdef\@journalshort{Polymers}	\gdef\@journalfull{Polymers}	\gdef\@doiabbr{polym}	\gdef\@ISSN{2073-4360}	}
\DeclareOption{polysaccharides}{	\gdef\@journal{polysaccharides}	\gdef\@journalshort{Polysaccharides}	\gdef\@journalfull{Polysaccharides}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{preprints}{ 	\gdef\@journal{preprints} 	\gdef\@journalshort{Preprints}	\gdef\@journalfull{Preprints}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{proceedings}{	\gdef\@journal{proceedings}	\gdef\@journalshort{Proceedings}	\gdef\@journalfull{Proceedings}	\gdef\@doiabbr{proceedings}	\gdef\@ISSN{2504-3900}	}
\DeclareOption{processes}{	\gdef\@journal{processes}	\gdef\@journalshort{Processes}	\gdef\@journalfull{Processes}	\gdef\@doiabbr{pr}	\gdef\@ISSN{2227-9717}	}
\DeclareOption{proteomes}{	\gdef\@journal{proteomes}	\gdef\@journalshort{Proteomes}	\gdef\@journalfull{Proteomes}	\gdef\@doiabbr{proteomes}	\gdef\@ISSN{2227-7382}	}
\DeclareOption{psych}{	\gdef\@journal{psych}	\gdef\@journalshort{Psych}	\gdef\@journalfull{Psych}	\gdef\@doiabbr{psych}	\gdef\@ISSN{2624-8611}	}
\DeclareOption{publications}{	\gdef\@journal{publications}	\gdef\@journalshort{Publications}	\gdef\@journalfull{Publications}	\gdef\@doiabbr{publications}	\gdef\@ISSN{2304-6775}	}
\DeclareOption{quantumrep}{	\gdef\@journal{quantumrep}	\gdef\@journalshort{Quantum Rep.}	\gdef\@journalfull{Quantum Reports}	\gdef\@doiabbr{quantum}	\gdef\@ISSN{2624-960X}	}
\DeclareOption{quaternary}{	\gdef\@journal{quaternary}	\gdef\@journalshort{Quaternary}	\gdef\@journalfull{Quaternary}	\gdef\@doiabbr{quat}	\gdef\@ISSN{2571-550X}	}
\DeclareOption{qubs}{	\gdef\@journal{qubs}	\gdef\@journalshort{Quantum Beam Sci.}	\gdef\@journalfull{Quantum Beam Science}	\gdef\@doiabbr{qubs}	\gdef\@ISSN{2412-382X}	}
\DeclareOption{reactions}{	\gdef\@journal{reactions}	\gdef\@journalshort{Reactions}	\gdef\@journalfull{Reactions}	\gdef\@doiabbr{reactions}	\gdef\@ISSN{2624-781X}	}
\DeclareOption{recycling}{	\gdef\@journal{recycling}	\gdef\@journalshort{Recycling}	\gdef\@journalfull{Recycling}	\gdef\@doiabbr{recycling}	\gdef\@ISSN{2313-4321}	}
\DeclareOption{religions}{	\gdef\@journal{religions}	\gdef\@journalshort{Religions}	\gdef\@journalfull{Religions}	\gdef\@doiabbr{rel}	\gdef\@ISSN{2077-1444}	}
\DeclareOption{remotesensing}{	\gdef\@journal{remotesensing}	\gdef\@journalshort{Remote Sens.}	\gdef\@journalfull{Remote Sensing}	\gdef\@doiabbr{rs}	\gdef\@ISSN{2072-4292}	}
\DeclareOption{reports}{	\gdef\@journal{reports}	\gdef\@journalshort{Reports}	\gdef\@journalfull{Reports}	\gdef\@doiabbr{reports}	\gdef\@ISSN{2571-841X}	}
\DeclareOption{resources}{	\gdef\@journal{resources}	\gdef\@journalshort{Resources}	\gdef\@journalfull{Resources}	\gdef\@doiabbr{resources}	\gdef\@ISSN{2079-9276}	}
\DeclareOption{risks}{	\gdef\@journal{risks}	\gdef\@journalshort{Risks}	\gdef\@journalfull{Risks}	\gdef\@doiabbr{risks}	\gdef\@ISSN{2227-9091}	}
\DeclareOption{robotics}{	\gdef\@journal{robotics}	\gdef\@journalshort{Robotics}	\gdef\@journalfull{Robotics}	\gdef\@doiabbr{robotics}	\gdef\@ISSN{2218-6581}	}
\DeclareOption{safety}{	\gdef\@journal{safety}	\gdef\@journalshort{Safety}	\gdef\@journalfull{Safety}	\gdef\@doiabbr{safety}	\gdef\@ISSN{2313-576X}	}
\DeclareOption{sci}{	\gdef\@journal{sci}	\gdef\@journalshort{Sci}	\gdef\@journalfull{Sci}	\gdef\@doiabbr{sci}	\gdef\@ISSN{2413-4155}	}
\DeclareOption{scipharm}{	\gdef\@journal{scipharm}	\gdef\@journalshort{Sci. Pharm.}	\gdef\@journalfull{Scientia Pharmaceutica}	\gdef\@doiabbr{scipharm}	\gdef\@ISSN{2218-0532}	}
\DeclareOption{sensors}{	\gdef\@journal{sensors}	\gdef\@journalshort{Sensors}	\gdef\@journalfull{Sensors}	\gdef\@doiabbr{s}	\gdef\@ISSN{1424-8220}	}
\DeclareOption{separations}{	\gdef\@journal{separations}	\gdef\@journalshort{Separations}	\gdef\@journalfull{Separations}	\gdef\@doiabbr{separations}	\gdef\@ISSN{2297-8739}	}
\DeclareOption{sexes}{	\gdef\@journal{sexes}	\gdef\@journalshort{Sexes}	\gdef\@journalfull{Sexes}	\gdef\@doiabbr{}	\gdef\@ISSN{2411-5118}	}
\DeclareOption{signals}{	\gdef\@journal{signals}	\gdef\@journalshort{Signals}	\gdef\@journalfull{Signals}	\gdef\@doiabbr{signals}	\gdef\@ISSN{2624-6120}	}
\DeclareOption{sinusitis}{	\gdef\@journal{sinusitis}	\gdef\@journalshort{Sinusitis}	\gdef\@journalfull{Sinusitis}	\gdef\@doiabbr{sinusitis}	\gdef\@ISSN{2309-107X}	}
\DeclareOption{smartcities}{	\gdef\@journal{smartcities}	\gdef\@journalshort{Smart Cities}	\gdef\@journalfull{Smart Cities}	\gdef\@doiabbr{smartcities}	\gdef\@ISSN{2624-6511}	}
\DeclareOption{sna}{	\gdef\@journal{sna}	\gdef\@journalshort{Sinusitis Asthma}	\gdef\@journalfull{Sinusitis and Asthma}	\gdef\@doiabbr{sna}	\gdef\@ISSN{2624-7003}	}
\DeclareOption{societies}{	\gdef\@journal{societies}	\gdef\@journalshort{Societies}	\gdef\@journalfull{Societies}	\gdef\@doiabbr{soc}	\gdef\@ISSN{2075-4698}	}
\DeclareOption{socsci}{	\gdef\@journal{socsci}	\gdef\@journalshort{Soc. Sci.}	\gdef\@journalfull{Social Sciences}	\gdef\@doiabbr{socsci}	\gdef\@ISSN{2076-0760}	}
\DeclareOption{soilsystems}{	\gdef\@journal{soilsystems}	\gdef\@journalshort{Soil Syst.}	\gdef\@journalfull{Soil Systems}	\gdef\@doiabbr{soilsystems}	\gdef\@ISSN{2571-8789}	}
\DeclareOption{sports}{	\gdef\@journal{sports}	\gdef\@journalshort{Sports}	\gdef\@journalfull{Sports}	\gdef\@doiabbr{sports}	\gdef\@ISSN{2075-4663}	}
\DeclareOption{standards}{	\gdef\@journal{standards}	\gdef\@journalshort{Standards}	\gdef\@journalfull{Standards}	\gdef\@doiabbr{}	\gdef\@ISSN{2305-6703}	}
\DeclareOption{stats}{	\gdef\@journal{stats}	\gdef\@journalshort{Stats}	\gdef\@journalfull{Stats}	\gdef\@doiabbr{stats}	\gdef\@ISSN{2571-905X}	}
\DeclareOption{surfaces}{	\gdef\@journal{surfaces}	\gdef\@journalshort{Surfaces}	\gdef\@journalfull{Surfaces}	\gdef\@doiabbr{surfaces}	\gdef\@ISSN{2571-9637}	}
\DeclareOption{surgeries}{	\gdef\@journal{surgeries}	\gdef\@journalshort{Surgeries}	\gdef\@journalfull{Surgeries}	\gdef\@doiabbr{}	\gdef\@ISSN{2017-2017}	}
\DeclareOption{sustainability}{	\gdef\@journal{sustainability}	\gdef\@journalshort{Sustainability}	\gdef\@journalfull{Sustainability}	\gdef\@doiabbr{su}	\gdef\@ISSN{2071-1050}	}
\DeclareOption{symmetry}{	\gdef\@journal{symmetry}	\gdef\@journalshort{Symmetry}	\gdef\@journalfull{Symmetry}	\gdef\@doiabbr{sym}	\gdef\@ISSN{2073-8994}	}
\DeclareOption{systems}{	\gdef\@journal{systems}	\gdef\@journalshort{Systems}	\gdef\@journalfull{Systems}	\gdef\@doiabbr{systems}	\gdef\@ISSN{2079-8954}	}
\DeclareOption{technologies}{	\gdef\@journal{technologies}	\gdef\@journalshort{Technologies}	\gdef\@journalfull{Technologies}	\gdef\@doiabbr{technologies}	\gdef\@ISSN{2227-7080}	}
\DeclareOption{test}{	\gdef\@journal{test}	\gdef\@journalshort{Test}	\gdef\@journalfull{Test}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{toxics}{	\gdef\@journal{toxics}	\gdef\@journalshort{Toxics}	\gdef\@journalfull{Toxics}	\gdef\@doiabbr{toxics}	\gdef\@ISSN{2305-6304}	}
\DeclareOption{toxins}{	\gdef\@journal{toxins}	\gdef\@journalshort{Toxins}	\gdef\@journalfull{Toxins}	\gdef\@doiabbr{toxins}	\gdef\@ISSN{2072-6651}	}
\DeclareOption{tropicalmed}{	\gdef\@journal{tropicalmed}	\gdef\@journalshort{Trop. Med. Infect. Dis.}	\gdef\@journalfull{Tropical Medicine and Infectious Disease}	\gdef\@doiabbr{tropicalmed}	\gdef\@ISSN{2414-6366}	}
\DeclareOption{universe}{	\gdef\@journal{universe}	\gdef\@journalshort{Universe}	\gdef\@journalfull{Universe}	\gdef\@doiabbr{universe}	\gdef\@ISSN{2218-1997}	}
\DeclareOption{urbansci}{	\gdef\@journal{urbansci}	\gdef\@journalshort{Urban Sci.}	\gdef\@journalfull{Urban Science}	\gdef\@doiabbr{urbansci}	\gdef\@ISSN{2413-8851}	}
\DeclareOption{vaccines}{	\gdef\@journal{vaccines}	\gdef\@journalshort{Vaccines}	\gdef\@journalfull{Vaccines}	\gdef\@doiabbr{vaccines}	\gdef\@ISSN{2076-393X}	}
\DeclareOption{vehicles}{	\gdef\@journal{vehicles}	\gdef\@journalshort{Vehicles}	\gdef\@journalfull{Vehicles}	\gdef\@doiabbr{vehicles}	\gdef\@ISSN{2624-8921}	}
\DeclareOption{vetsci}{	\gdef\@journal{vetsci}	\gdef\@journalshort{Vet. Sci.}	\gdef\@journalfull{Veterinary Sciences}	\gdef\@doiabbr{vetsci}	\gdef\@ISSN{2306-7381}	}
\DeclareOption{vibration}{	\gdef\@journal{vibration}	\gdef\@journalshort{Vibration}	\gdef\@journalfull{Vibration}	\gdef\@doiabbr{vibration}	\gdef\@ISSN{2571-631X}	}
\DeclareOption{viruses}{	\gdef\@journal{viruses}	\gdef\@journalshort{Viruses}	\gdef\@journalfull{Viruses}	\gdef\@doiabbr{v}	\gdef\@ISSN{1999-4915}	}
\DeclareOption{vision}{	\gdef\@journal{vision}	\gdef\@journalshort{Vision}	\gdef\@journalfull{Vision}	\gdef\@doiabbr{vision}	\gdef\@ISSN{2411-5150}	}
\DeclareOption{water}{	\gdef\@journal{water}	\gdef\@journalshort{Water}	\gdef\@journalfull{Water}	\gdef\@doiabbr{w}	\gdef\@ISSN{2073-4441}	}
\DeclareOption{wem}{	\gdef\@journal{wem}	\gdef\@journalshort{Wildl. Ecol. Manag.}	\gdef\@journalfull{Wildlife Ecology and Management}	\gdef\@doiabbr{}	\gdef\@ISSN{1234-4321}	}
\DeclareOption{wevj}{	\gdef\@journal{wevj}	\gdef\@journalshort{World Electric Vehicle Journal}	\gdef\@journalfull{World Electric Vehicle Journal}	\gdef\@doiabbr{wevj}	\gdef\@ISSN{2032-6653}	}

==> proposals and backups/1-introduction_frame.tex <==
\section{Introduction}


Task-oriented dialog systems: 
    need to link knowledge representation to user input
    Grammar preparation require expertise and human labour in domain engineering 
    Therefore, approaches automating the process has been being proposed, but requires high volume of labelled data, and many models are blackbox, which affects the implementation where insights into the inner working of model is required
Previously proposed:
    CPM can extract key concepts in the text (topic)
    CPM also demonstrated potential in extracting semantic structure by processing the properties of convex polytope
    Now, will discuss how to utilize the properties and how to interpret them in NLU models
Problem statement:
    As an extension to our previous finding, This paper will discuss several ways demonstrate how CPM can assist in NLU with limited labelled data and improve model interpreability by deriving semantic information from geometric properties in convex polytope
Contribution
    \begin{enumerate}
        \item we propose an unsupervised method via CPM to automatically extract key semantic features with high interpretability from raw conversation data (copied from iscslp paper)
        \item we discuss how to interpret the extracted semantic features derived from CPM properties in NLU model; 
        % find CPM 
        \item we demonstrate that CPM can assist in boosting the performance in NLU models with limited labelled data and provide interpretability 
        %modify this according to our actual experiment
    \end{enumerate}
    

==> proposals and backups/1-introduction_no_ontology.tex <==
\section{Introduction}

Task-oriented dialog system is receiving increasing attention in both research and industrial community.  It can serve as a natural interface to help users achieve certain goals through natural conversation and has been adopted to many applications such as personal assistant, e-commerce sales assistant, etc.

To assist users to accomplish certain tasks, the system needs to understand the user’s utterances and extract necessary information from them, where the process is usually referred to as Natural Language Understanding (NLU).
The extracted information is commonly represented by a structured form called \textit{semantic frame}, which involves intent and a set of semantic roles. Intent refers to goals of user queries, and certain words in the queries have specific semantic roles related to the intent, categorized using slot labels.  Fig. \ref{fig:frame-example} shows an example of a well-labeled user utterance from Air Travel information Systems (ATIS) dataset \citep{price1990evaluation}, `What flights are there on Sunday from Seattle to Chicago', and its corresponding semantic frame `Flights(Origin=Seattle, Destination=Chicago, Date=Sunday)'. In this example, the word "Sunday" is the date attribute of the query subject "flight" that is the intent of this utterance, and this semantic relation is referred to as "semantic roles". Understanding the utterance requires determining its intent and identify the intent-related semantic roles of all words in the utterance. In NLU tasks, this is equivalently done by classifying words and utterances the into slot and intent labels, respectively.

Note that for a certain domain, such as the air travel information domain of ATIS, the possible number of categories of intents and slots are usually finite but may vary in size due to extension of domain.
 \input{tables/fig:frame}
 
A common approach to achieve NLU is rule-based method, where domain experts are employed to design a set of heuristic parsing rules to locate slots and intents, and model the utterances \citep{saini2019linguistic}. 
However, the grammar rules have limitation in modeling the complex structures of real-world dialog as they are simply based on syntactic knowledge of the utterances, and a complex dialog system may require a large number of rules to model which is difficult to design manually. 
Another popular approach is machine learning-based NLU  \citep{firdaus2020deep, liu2016attention, chen2016knowledge} which requires a huge amount of training data of utterances with well-labeled intents and slots-value pairs for supervised learning.
Although the neural-based supervised learning model has achieved state-of-the-art NLU performance, it acts like a black-box which shows limited clues on the reasoning process in filling the semantic frame. Note that both mentioned approaches require experts either to design the parsing rules or to label the training data, which are labor-intensive and thus costly. Besides, they are not adaptive to domain extension especially when the domain changes actively in time.
This paper presents an alternative approach that functions by summarizing and utilizing semantic structures from dialog interaction data, which only requires a corpus of sentences or transcribed utterances with minimal labeling.  This is aimed to facilitate natural language understanding with little supervision. 
We observe that in task-oriented dialogues, certain word patterns (e.g. phrases) that appear frequently tend to anticipate the information related to various INTENTS and SLOTS. 
Syntactically, lexical components as slot values and intents could either precede or succeed such word patterns, but not necessarily immediately.
For example, in the ATIS corpus, the ORIGIN slot usually appears in the user’s query in the format of ‘from CITY-NAME’, e.g. from San Francisco.
We define "semantic patterns" as slot and intents, their depending word patterns, and the syntactical relations between them.  
Hence, we can leverage such semantic patterns in identifying the presence of intents and the slot labels of words. Furthermore, we also notice that a sentence/utterance is usually composed of several patterns, e.g., a user’s query for search flights usually contains a combination of patterns related to the INTENT (i.e. FINDFLIGHT) and SLOTS (e.g. ORIGIN, DESTINATION, DATE AND TIME). 
%The objective is to identify the possible sets of INTENTS and information SLOTS that need to be filled into the semantic frame (as shown in the lower part of Fig. \ref{fig:frame-example}).
This paper proposes the Convex Polytopic Model (CPM) \citep{wu2018topic}, which offers a data-driven, unsupervised yet interpretable framework that can (i) automatically discover potential semantic patterns by analyzing raw dialog data; (ii) facilitate analyses and visualization of the underlying semantics structures 
and (iii) allow injection of CPM features into a neural-based model such that the knowledge incorporated can help lower the requirements of labeled training data.

CPM is an unsupervised geometric algorithm that can extract the key semantic concepts from corpora of short texts \citep{wu2018topic}, which was previous applied to the discovery of information topics from a corpus of short documents. This paper applies a similar algorithm to the utterances from a dialog corpus by first projecting the utterances to a low-dimensional affine subspace via Principal Component Analysis (PCA), and then enclosing the projected points within a compact convex polytope. The CPM algorithm can effectively discover the semantic patterns (exhibited as the polytope vertices) that are closely related to the semantic frame and can simultaneously decompose all utterances in the dataset into combinations of the semantic patterns.
We apply CPM on the ATIS dataset to demonstrate its ability in extracting useful features for achieving NLU. 
First, we show that the polytope vertices are closely related to the semantic patterns by comparing the results with human-labeled data.
Second, we analyze the semantic structure of individual utterance from two perspectives: 
(i) \textit{compositional analysis}: as each utterance point in the polytope can be represented as a convex combination of vertices, the combination coefficients can thus reveal the composition ratio of the semantic patterns within the utterance; 
(ii) \textit{word-word correlation analysis}: the word-word correlation within the utterance can be discovered based on the word vectors using semantic patterns as the features, which reveals the internal semantic structure . 
Third, we further incorporate the CPM-discovered features to guide the neural-based model in the example task of slot filling, where we show that such incorporation can achieve significantly better performance when have less labeled data.
Our contributions are three-fold: 
1) we propose a novel, unsupervised method via CPM to summarize semantic patterns in task-oriented dialog corpus and discover the underlying semantic structure in the utterances; 
2) we demonstrate the high interpretability and transparency of the CPM model via various visualization techniques; 
3) we verify that CPM extracted features can boost the performance of the NLU models in limited labeled data cases while enhancing the interpretability of the neural-based models for slot filling.

==> proposals and backups/1-introduction_v1.tex <==
\section{Introduction}

Task oriented dialog system is receiving increasing attention in both research and industrial community.  It can serve as a natural interface to help users achieve certain goals through natural conversation and has been adopted to many applications such as personal assistant, e-commerce sales assistant, etc. .
%ontology is needed

To build a task-oriented dialog system from scratch, the initial step is to clarify the targeted tasks and design the domain ontology (ref). For example, a flight booking assistant should be able to handle tasks including \textit{flight information query, airfare query}, etc., which are also referred to as user \textit{intents}. 
The ontology of the domain consists of not only possible user intents, but also the related attributes (\textit{slots} with values). 
For example, Fig. \ref{fig:frame-example} shows a well labeled user utterance from Air Travel information Systems (ATIS) dataset, ``What flights are there on Sunday from Seattle to Chicago”, and its corresponding semantic frame (consisting of intent and corresponding slots) ``Flights(Origin=Seattle, Destination=Chicago, Date=Sunday)”.
\input{tables/fig:frame} 
The design of ontology also defines the scope of the conversations between users and the system. 
%ontology is typically handcrafted
A typical approach is to employ domain experts to define the ontology and design a set of heuristic rules to model the dialog and understand user's input via parser (ref), which is a laborious process and restricts the flexibility of dialog system development.
%nlu models are obscure and cannot take unlabelled data
Approaching this problem in another direction, many current dialog system researches assume that the ontology is already given (by the labeled data) and focus on improving the performance of the modularized dialog system via supervised training which requires a lot of well-labeled data. 
An important component  of such systems is natural language understanding (NLU) which aims to .
Unfortunately, the lack of well-labeled conversational data and low interpretability of such models have been bottlenecks in dialog system development. Also, this assumption ignores the ontology discovery procedure and results in great obstacles in adapting a dialog system to different domains.  
%A more practical

Nowadays, we already have numerous unlabeled human-human or human-computer conversational log in many domains. These data can roughly cover the scope of the domain. \textcolor{red}{Therefore, we aim to utilize the unlabeled data for \textit{automatic ontology discovery} and fill the gap between ontology discovery and the language understanding task in the dialog system development.}
%...?
[This paragraph summarizes the intent mining works, Need Refinement] Focusing on exploiting raw conversational data, (Ref1, Perkins 2019 ) , (Ref2, Chatterjee 2020), and (Ref3, Haponchyk 2018) utilize clustering algorithms to implement an expert-in-the-loop method to assist labelling work. They requires some seed data and the results are efficacy but noisy. (Ref4, Mallinar 2018) aims to provide a more human-friendly interface for expert annotators and adopts data programming techniques to expand the labels to more data. These approaches are all trying to produce more intent-related clusters by improving the representations of the intent-level semantics of the user queries. Also, all of these works focus on intent mining. However, both the the intent and slots are of great importance for understanding user's query. 
%human understanding of language involve "linguistic features"
And for the language understanding task, although the inputs are sequences of words, a natural way for a human participant to understand them is to reconstruct the rich underlying linguistic structures that help the participant capture the key information and relations between them (better use a figure to illustrate this point) (ref mannings, 2020). 
%other approahes are not insightful and interpretable
The rule-based systems recover the underlying linguistic structure by handcrafted grammar rules, which requires heavy engineering work and is hard to generalize. Also, the rules are usually highly related to syntax knowledge, but not essentially to the semantic information. 
While the popular neural approaches have no concern on approximating the nature of human understanding and consider the task as transform user’s input into a task-specific semantic frame. Specifically, these systems usually contain  an utterance class classification task for intent identification and a sequence labelling task for slot-filling. These approaches that achieve the state-of-the-art performance on these tasks with a huge amount of well labeled data, but lacks of interpretability and provides no insight regrading how these knowledge are learnt by human.

Considering the two issues above, we propose an unsupervised, data-driven, interpretable framework to discover the domain ontology by exploiting the raw conversational data (exp1.1, 1.2), approximate human understanding procedure to analyze the underlying semantic structure in user utterances(exp1.3), and assist NLU tasks by injecting semantic frame features and increasing the interpretability(exp2). 
%finding semantic structure through patterns
As mentioned before, this work mimic the human behavior of language understanding: extracting key information and constructing the links among the information.
In the task-oriented dialog corpus, there are many certain kind of patterns that repeatedly occurring in the corpus. Usually these patterns indicate the intent and slots information. For example, in ATIS dataset, the \textit{Origin} slot is summarized by a pattern ``from \textit{city-name}'', e.g. ``from San Francisco''. 
Hence, semantic patterns serve as the key components of the corpus and are critical features for the domain ontology discovery in task-oriented dialog system.  
Additionally, user queries are composed of such patterns: a user query that looking for flights usually contains patterns that exhibit \textit{Find flight, Origin, Destination, Time} information.

Therefore, we present this work which can 1) unmix those patterns from the corpus (exp 1.1), 2) reveal the compositional relation between each utterance and the semantic patterns (exp 1.2), and 3) approximate the human understanding procedure and reconstruct each utterance's semantic structure (exp 1.3).

Specifically, we utilize the Convex Polytopic Model(CPM) (ref) that enclose all the PCA-projected utterance points with a compact convex polytope to model the dialog corpus and interpret the geometric features for understanding. CPM is an unsupervised algorithm proposed by Wu et al. in (ref) that can extract the critical concepts in the corpus of short texts. For example, in (ref), it is utilized for discovering topics from a set of documents that have mixture of topics. 

In this paper, we show that the geometric properties of the polytope are closely related to the semantic patterns that indicate slot-value pairs and intents in the corpus. We also visualize the underlying semantic structure in the utterances interpreted from the algebraic result of CPM.
Then we utilize CPM extracted semantic features to guide SOTA neural-network-based approaches for slot filling and intent classification tasks. The result shows that the CPM extracted features can not only introduce interpretability to the model, but also significantly improve its performance with limited well-labelled training data. 

In this paper, we show that the vertices of the polytope are closely related to the semantic patterns that indicate slot-value pairs and intents in the corpus. We also visualize the semantic pattern composition and underlying semantic structure in the utterances interpreted from the algebraic result of CPM.


The CPM extracted semantic knowledge can be used to guide SOTA neural-network-based approaches for slot filling and intent classification tasks. Our experiment shows that the extracted features can not only introduce interpretability to the model, but also significantly improve its performance with limited well-labelled training data. 
This framework can also be integrated to the expert-in-the-loop systems to facilitate the labeling procedure of training set mentioned above.

Our contribution is three-fold: 
1) We introduce and analyse the nature of human understanding for NLU task in the conversational system and approximate the procedure by a data-driven framework.
2) we propose a novel, unsupervised method via CPM to exploit domain ontology in task-oriented dialog corpus and discover the underlying semantic structure in the utterances; 
3) we demonstrate the high interpretability and transparency of our model; 
4) we show CPM extracted features enhance interpretability of the deep learning models for NLU tasks and boost the performance of the NLU models providing limited labelled data.

%Proposed change: Our contribution is three-fold: 1) we propose a novel, unsupervised method via CPM to extract recurring semantic patterns that are a set of coherent structures related underlying semantic frames. 2) we demonstrate the high interpretability and transparency of our model; 3) we show CPM extracted features enhance interpretability of the deep learning models for NLU tasks and boost the performance of the NLU models providing limited labelled data through the understanding of utterances. 

==> proposals and backups/3-methodology_frame.tex <==
\section{Methodology}

% Consider

% \textbf{Notes:}
% \begin{enumerate}
%     \item be aware of geometric proprieties and linguistic properties.
%     \item  use a fake dataset for illustration?
% \end{enumerate}
\subsection{detailed structure}
    \\CPM steps:
    \begin{enumerate}
        \item pre-processing utterances (ignore)
        \item   utterances -sum-normalized TDM->points . This step introduces following properties:
        \begin{enumerate}
            
            \item The utterances are first transformed into a sum-normalized TDM and X, where the $X_ij$ is the frequency of the $i-$th term in the $j-$th utterance. And the \textbf{Euclidean distances} between data points measures the distances between them.  (\textcolor{red}{[Experiment 1? : show that the closer the utterance points are, the more similar they are to each other})
            
            \item the utterances that contain fewer semantic patterns tend to be the extreme points (i.e. lie further away from the centre of the hyperplane).  (\textcolor{red}{Experiment 2? : show some furthest utterance points (preliminary result: ``what is aircode?";``"show flights from city name to city name"} )
        \end{enumerate}
        
        \item Embed the utterance points onto a lower dimensional subspace: points -PCA-> a lower-dimensional subspace. [Reason for PCA, not certain] Finding convex polytope on the original high dimension subspace is not a trivial work. Therefore, we aim to find a closest low-dimensional subspace for the utterance points. \textcolor{green}{Example 1: point set}   % what if no PCA? like on a small corpus, directly find convex polytope?
        
        This step introduces following properties:
            \begin{enumerate}
                \item PCA finds the principle components that corresponds to the direction where the data has the largest variance. and we will find the compact convex polytope on this lower-dimensional subspace. 
                \item As PCA preserves the distinctive features of the utterance points, the extreme points remain extreme after PCA projection. Higher dimension preserves more features
                %\item Note that not all the extreme points remains extreme now, as some features are compressed. Therefore, the features founded by CPM is filtered by PCA 
            \end{enumerate}
            %[No Need to mention properties of the principle compoents, as we are not going to use it] \item Question : what are the PCA components? :   are fitted into the R-D ellipsoid, the axes of the ellipsoid are principal components -> data has largest variance along which direction (most distinguishable features) -> \textcolor{red}{Assumption missing here, e.g., on linguistic level, semantic patterns are the features that distinguishes the corpus} ->
        
        \item Generate a compact convex polytope to enclose the embedded utterances
        There are several ways to generate a convex polytope.
        \begin{enumerate}
            \item NO-type [pros: minimal volume]: here we should use example to validate this framework (in the assumption section) \textcolor{green}{Example 2: NO};  \textcolor{red}{Experiment  3: a. Scope? [experiment can be done using DSTC dataset] b. Patterns? }
            \item MVS-type [pros: extract patterns from corpus]:\textcolor{green}{Example 3: 2D MVS} \textcolor{red}{Experiment 4: 2D MVS}  Also, here we should mention how to interpret vertices:
            \begin{enumerate}
            \item directly using coordinates: utterance = composition of semantic concepts embedding (convex representation directly fed to neural network) 
            \item  on the original TDM-spanned space: coordinates -> topwords (related to pattern and chaining) or coordinates -> token importance to vertices (attention) \textcolor{red}{Experiment 5: token representation (attention heat map)}
                \item euclidean distances (k-means) (knn) \textcolor{red}{Experiment 6: pattern formation and comparing to Stanford parser}
         \end{enumerate}
     
            % what does the previously found 2D type polytope looks like on the 3D subspace?}
        \end{enumerate}
    \end{enumerate}

% \subsection{Convex Polytopic Model}
%     In this section, we will explain the detailed steps of CPM, along with resulting properties and illustrative examples. 
%     CPM involves two major steps. First, the utterances are embedded into a low-dimensional affine subspace by Principal Component Analysis (PCA). 
    
%     Second, A convex polytope is subsequently computed, enclosing all embedded utterance points in the subspace. 
    
    
%     a. PCA
%     The utterances are first prepared as a term-document matrix, where (describe tdm). 
%     Given that we need to extract a limited number of latent features, and the vocabulary size of TDM is usually very large, we perform PCA to reduce the dimension of the vector representation of utterances. (why pca)
    % Additionally, due to the potential inequality of word count in different utterances, the subspace vector of PCA can only be compared by cosine similarity, while word count in utterances influence the norm and the euclidean distance between projected points cannot be used. This can be solved by performing sum-normalization across columns of tdm (i.e. individual utterances) to ensure that the tdm is on a sum-to-one hyperplane. (Why sum-normalization)
%     The pca can then be performed by eigenvaue decomposition on the covariance matrix of the sum-normalized tdm.
%     This is in contrast to traditional lsa where no normalization is pre-applied and the result can only be utlized through cosine similarity. The result are utterance points projected to low dimensional space, with the dataset having largest variance along the principle components. (expand a little bit here with the description above)
%     (example: correlation matrix of lsa and pca on the dataset. expect to see that first component of lsa is somewhat related to other components, while not obvious in the pca, which is desired since we are not wasting components)
%     b. NO/MVS
%   While the basis of pca can be interpreted as latent features in the corpus, the coefficients of such features (i.e. coordinates of points) are not bounded in non-negative real number space, which renders the explanation more difficult, since we want to decompose linguistic concepts to utterances, and it is hard to imagine a concept "negatively contributing" to the utterance. We therefore favor a new basis, on top of which all points are the convex combination of the basis vectors. 
   
%   As discussed above, distance between points in the affine subspace is meaningful in describing the similarity between utterances. Following the idea, points at the edge of the utterances set are relatively different to other utterances. If we find the convex set enclosing the utterance points, we can describe any utterance points in the set with at least dimension+1 points in the hull, and to capture the unique concepts, the points should be chosen in the extreme set of such convex hull. To describe the corpus with a set of unique concepts that are still relevant to the utterances, i.e. as close as possible to the utterances points set, we need to find the convex hull of the utt points set. This could be performed using (introduce no and mvs)
%   (explain the difference between no and mvs)
%   (explain mvs algorithm)
% \subsection{Properties}
%     \begin{enumerate}
%         \item utterances are projected to subspace; utterance consisting of concepts of multiple vertices = interior
%         \item vertices capture distinct semantic concepts, which could be derived from the following properties:
%         \begin{enumerate}
%             \item  - projecting back to original tdm-spanned space: coordinates -> topwords (related to pattern and chaining) or coordinates -> token importance to vertices (attention)
%         \item directly using coordinates: utterance = composition of semantic concepts embedding (convex representation directly fed to neural network)
%         \item euclidean distances (k-means) (knn)
%         \end{enumerate}
%     \end{enumerate}


==> proposals and backups/backup.tex <==
%%%%%%%%% Experiment%%%%%%%%%%5

(mvs polytope -> close distance between vertex and extreme points -> similar concepts)
(correlation matrix of vertices in no and mvs separately -> similar concept illustrated by topwords ~ higher correlation) 
(pick utterance near edge and in center, show their word sequence + combination coefficients, compare with the vertices in NO and MVS -> points are convex comb of vertices ~ utterances are comb of captured concepts; mvs more distinct)

(high dim polytope captures more distinct concept, visualized by topwords; concept in low dim vertex split into multiple vertices in high dim)
(repeat the last experiment above: vertices that does not change a lot observe little coefficient change; vertices that are split going to high dim polytope see the coefficients distributed to the new vertices, more or less)


%Brief introduction of what we are going to do with the features

%\subsection{Applications}
%\subsubsection{Application 1. semantic pattern generation}
%\textcolor{red}{Experiment 6}
%topwords frequently appear in the corpus (show appearance count); (draw vocabulary distribution; compare the distributions) recurrent appearance = importance -- "knowledge substructure" (if show parser comparison below) / "grammar" (if show annotation result below)

%topwords co-exist in utterances; pattern with high coefficient about a vertex have topwords appear in it; (show examples here or link to above subsections)
%Chaining two topwords together generates patterns that are also frequently appear in patterns (show stats), pointing to important locations related to the semantic frame. (show examples, compare with parsers result if any)
%(plug the patterns in vivian k-san model and compare performance if possible - cpm can find knowledge substructure usable in nlu tasks)
% vertices - topwords - patterns - linguistic structure (or whatever notation used by the parser) chain established
%verified property: 2.1
% \subsubsection{Application 2.knowledge-guided attention}
%For structure in this section, refer to the Bahdanau attention paper 

==> proposals and backups/body.tex <==
\section{Formulation of CPM}

The process of CPM consists of three basic steps: 1) Represent each utterance in the dialog corpus by a sum-normalized term frequency vector; 2) Project all the utterance vectors onto a low-dimensional affine subspace via Principal Component Analysis (PCA); and 3) Generate a Minimum Volume Simplex (MVS), a special type of convex polytope, to enclose the projected utterances. The details of each step will be explained in the following subsections.

\noindent\textbf{Step 1: Representing each utterance as sum-normalized term frequency vector}

Given a task-oriented dialog corpus of $M$ utterances, we pre-process it by removing the stopwords and build a vocabulary of size $N$. We then represent each utterance by an $N$ dimensional vector with each entry as the occurrence count of the corresponding word divided by the total number of words, which is referred as sum-normalized term frequency vector where its sum equals one. The term frequency vector has traditionally been applied as document representation in natural language processing and information retrieval. Such representation discards the grammar and word order and is thus expected to preserve the semantics of the document. We therefore expect that in the use case of dialog corpus, it can also preserve the semantics of the utterance.

Geometrically, the utterance vector can be considered as a point on a $(N-1)$-dimensional sum-to-one hyperplane in the nonnegative orthant of the $N$-dimensional space. Note that the sum-to-one hyperplane in the nonnegative orthant forms an $(N-1)$-dimensional regular simplex with vertices on the axes and the mean position of all the vertices as the vertex centroid, denoted as $c_s$ here. As the vector entry is computed by dividing the total number of words, shorter utterance vector tends to be sparser and with non-zero entries having larger values, and hence its associated point tends to be farther from $c_s$. Besides, the Euclidean distance between two utterance points characterizes the difference in semantics between their corresponding utterances as the utterances with similar semantics usually appear to have more overlapping words and thus the difference between their vectors is also smaller.

\noindent\textbf{Step 2: Project utterance vectors onto a low-dimensional affine subspace via PCA}

We aim to capture the important semantic information for building semantic frame by filtering out less important features, i.e. the values (e.g. Sunday/Monday/…) in slot-value pairs (e.g. weekday:Sunday/Monday/…) has little effect on the structure of a semantic frame, hence we propose to remove the components with little effect using PCA by discarding the small principal components. It is geometrically equivalent embedding the utterances into a low-dimensional affine subspace spanned by the principal axes computed by PCA. The process of PCA reduces the dimensionality by maximizing the variance which preserves large pairwise distances and thus the important semantic features (i.e. distinguishable features) of the utterances can remain in the projected points. We refer these points as \textit{projected utterance points} to distinguish from the original utterance points represented by the term frequency vector in Step 1.

Mathematically, the PCA process can be formulated as follows: We stack all the term utterance (column) vectors in the corpus to form a term-utterance matrix $\matr{X}\in\mathbb{R}^{N\times M}$. Let $\bar{\matr{X}}\in\mathbb{R}^{N\times M}$ be the matrix with each column equal the average of all the columns of $\matr{X}$. Then, we apply Singular Value Decomposition (SVD) to find the closest $R$-dimensional subspace that approximate $(\matr{X}-\bar{\matr{X}})$, where $R$ is the dimension of the low-dimensional subspace. By keeping the first $R$ eigenvectors of $(\matr{X}-\bar{\matr{X}})(\matr{X}-\bar{\matr{X}})^\transpose$, we obtain an orthonormal basis $\matr{U}\in\mathbb{R}^{N\times R}$. The utterance vectors can then be projected onto the $R$-dimensional utterance subspace spanned by the basis $\matr{U}$. The projected utterance points, denoted by $\{\matr{p}_i\}^M_{i=1}$, can thus be computed by the following formula:
%
\begin{equation}
	\label{eq:P}
    \matr{P} = \bar{\matr{X}} + \matr{U}\matr{U}^\transpose (\matr{X}-\bar{\matr{X}}).
\end{equation}
%
where the $\{\matr{p}_i\}^M_{i=1}$ are the columns of $\matr{P}\in\mathbb{R}^{N\times M}$. Note that the columns of $\matr{P}$ are still \textit{sum-to-one}, and consequently, the \textit{utterance points} are still on the \textit{sum-to-one hyperplane}.

We emphasis here the difference of the proposed PCA projection from the traditional algorithm of Latent Semantic Analysis (LSA) applied in information retrieval. In PCA, we aim to find the axes of an ellipsoid as the principal components by fitting the original utterance points in $\matr{X}$ into an $R$-dimensional ellipsoid. Note that the subspace spanned by the principal component axes is an affine subspace as we have subtracted $\matr{X}$ by its average $\bar{\matr{X}}$. However in LSA, the matrix $\matr{X}$ is neither sum-normalized nor subtracted by the average, and hence latent semantic space obtained by LSA is not an affine subspace. The key difference between our \textit{affine utterance subspace} and the \textit{latent semantic space} is that the former measures the difference of utterances by the spatial distance of their utterance points, while the latter measures with their included angle. We will show how such feature of affine utterance subspace is useful for finding meaning features for the dialog corpus in the next step.

From linguistic perspective, the semantics of the utterance can be represented by the \textit{semantic frame} which is characterized by the intent and slot-value pairs. As the process of PCA preserves the important semantics in utterance, we expect that the resulting utterance points can distinguish the difference in the semantic frames of the utterances.

\noindent\textbf{Step 3: Generate a Minimum Volume Simplex (MVS) to enclose the projected utterance points}

Although the PCA can preserve the most important semantics of a given corpus, the principal component axes may not be directly associated to linguistic concepts and thus uninterpretable, due to their orthogonal property. Hence, we aim to extract the semantic features that can be interpretable from the projected utterance points based on the geometric properties. As we know that the intent and slots in the semantic frames can characterize the utterances, and they represent certain kind of patterns that repeatedly occurring in the task-oriented dialog corpus, we propose to apply the MVS algorithm to extract such semantic patterns as the interpretable features. This is motivated by the observation that a semantic frame is usually a combination of \textit{semantic patterns} commonly sharded across different semantic frames. For example, the slot of destination (as a kind of semantic pattern) usually appears in the semantic frame in both looking for flights and asking about the airfare. Hence, they serve as the elementary components of the semantic frames. 

To represent such combination in the mathematical way, we attempt to represent each \textit{projected utterance point} (representing an utterance in the corpus) by a \textit{unique} convex combination of the \textit{semantic patterns}. Geometrically, it is equivalent to generating a simplex to enclose all the projected utterance points, as any point within the simplex can be uniquely represented by a convex combination of the simplex vertices. In this case, the simplex vertices can thus be considered as the representations of the \textit{semantic patterns}. However, there can be infinite many possible choices of enclosing simplex for a point set. Hence, we need to set a certain constraint to ensure the semantic patterns captured by the vertices are meaningful. We propose to apply the minimum volume constraint to best fit the finite region occupied by the finite set of projected utterance points. This is to guarantee the simplex to cover as little as possible the out-of-scope region of the given corpus, while fully covering the scope within the corpus. Note that a simplex in $R$-dimensional space has a fixed number of vertices of $R+1$ which means that the dimension of the affine subspace obtained by PCA controls the number of \textit{semantic patterns} extracted. The details of the MVS formulation will be discussed in the next section.

The reason for choosing the convex combination approach instead of the conventional clustering methods to extract interpretable semantic patterns is in two-fold. First, the clustering methods which try to cluster points with similar features usually do not effectively take into account the combination property of semantic patterns that exhibits in the utterances of the task-oriented dialog corpus. Second, as mentioned in Step 1, the sum-normalization forces the shorter utterance to be farther from the centre, and shorter utterance tends to have fewer semantic patterns (or possibly just a pure pattern). Hence, the semantic patterns should be lying around peripheral region or even outside the point set. Note that in Step 2, for the projected points in the peripheral region, its associated utterance also lies in the peripheral region before projection (but not vice versa). Therefore, it is reasonable to apply the convex combination approach to obtain the simplex such that the simplex vertices act as the extreme points that capture the pure semantic patterns.

\section{Minimum Volume Simplex Analysis}

This section describes the detailed formulation of MVS approach by first introducing the convex polytopic representation and then formulating the optimization problem of finding the MVS.

\subsection{Convex Polytopic Representation}

The \textit{convex polytopic representation} of the \textit{projected utterance point} $\matr{p}_i$ is defined as the convex combinations of $\matr{v}_j$:
%
\begin{equation}
	\label{eq:eq1}
    \matr{p}_i=\sum_{j=1}^K a_{ij} \matr{v}_j,
\end{equation}
%
Where $K$ is the number of vertices of the convex polytope and $a_{ij}\geq 0$ (non-negativity condition) and $\sum_{j=1}^K a_{ij}=1$ (sum-to-one condition), for $i=1, \ldots, M$, are the convexity conditions. For all the points $\{\matr{p}_i\}^M_{i=1}$ from the corpus enclosed by a convex polytope with vertices $\{\matr{v}_j\in\mathbb{R}^N\}^K_{j=1}$, (\ref{eq:eq1}) can thus be written in matrix form:
%
\begin{equation}
	\label{eq:eq2}
    \matr{P}=\matr{V}\matr{A},
\end{equation}
%
where $\{\matr{v}_j\}^K_{j=1}$ form the columns of $\matr{V}\in\mathbb{R}^{M\times K}$ and $\matr{A}\in\mathbb{R}^{K\times M}$ with entries $a_{ij}$. Note that all columns of $\matr{A}$, denoted by $\matr{a}_1, \ldots, \matr{a}_M$, are sum-to-one and non-negative.

\subsection{Finding MVS as an Optimization Problem}

To generate the MVS enclosing a point set lying on a $R$-dimensional subspace, we can formulate it as an optimization problem using the convex polytopic representation. Note that the number of vertices in the MVS $K=R+1$. Consider the projected utterance points of matrix $\matr{P}$ is known, we apply the algorithm originally proposed by Li et al. in \cite{li2008minimum,li2015minimum} to find the MVS. The MVS optimization problem can be expressed as follows:
%
\begin{equation}
	\label{eq:eq3}
    \textbf{P}=\textbf{VA} \quad s.t. \quad \textbf{A} \succeq 0 \quad and \quad \textbf{1}_K^\transpose \textbf{A}=\textbf{1}_M^\transpose
\end{equation}
%
where $\textbf{1}_K$ denotes the column vector of dimension $K$ with all entries equal \textit{one}.

Denote $\tilde{\textbf{P}}\in\mathbb{R}^{K\times M}$ and $\tilde{\textbf{V}}\in\mathbb{R}^{K\times K}$ as the projected version of $\matr{P}$ and $\matr{V}$, respectively. We define the projection matrix $\tilde{\textbf{U}}= [\matr{U}\; \matr{u_{orth}}]\in\mathbb{R}^{N\times K}$, where $\matr{u_{orth}}$ is the orthonormal component of the mean of $\matr{X}$ (denoted here by $\bar{\matr{x}}$) which can be calculated by $\matr{u_{orth}}=\matr{u_0}/\|\matr{u_0}\|$ where $\matr{u_0}=\bar{\matr{x}}-\matr{U}\matr{U}^\transpose \bar{\matr{x}}$. Hence, $\tilde{\textbf{P}}=\tilde{\textbf{U}}^\transpose\matr{P}$ and $\tilde{\textbf{V}}=\tilde{\textbf{U}}^\transpose\matr{V}$.

It is known that the volume of simplex confined by the origin and the columns of $\tilde{\textbf{V}}$ can be computed by $\left|\det(\tilde{\textbf{V}})\right|$, where $\det(\tilde{\textbf{V}})$ is the determinant of $\tilde{\textbf{V}}$. As the distance from the origin to the \textit{sum-to-one hyperplane} is fixed, minimizing the volume of simplex that contains all \textit{utterance points} is equivalent to minimizing the volume of simplex defined by the origin and the columns of $\tilde{\textbf{V}}$, the MVS problem can thus be formulated as follows:
%
\begin{equation}
	\label{eq:eq5}
	\begin{split}
	    \tilde{\textbf{V}}^* = &\argmin_{\tilde{\textbf{V}}} \left|\det(\tilde{\textbf{V}})\right|\\
	    s.t. \quad \tilde{\textbf{V}}^{-1}\tilde{\textbf{P}} \succeq 0& \quad and \quad \textbf{1}_K^\transpose \tilde{\textbf{V}}^{-1}\tilde{\textbf{P}}=\textbf{1}_M^\transpose.
	\end{split}
\end{equation}

Let $\matr{Q}\equiv\tilde{\textbf{V}}^{-1}$, we have $det(\matr{Q})=1/det(\tilde{\textbf{V}}$. The optimization problem (\ref{eq:eq5}) can then be written as follows:
%
\begin{equation}
	\label{eq:eq6}
	\begin{split}
	    \textbf{Q}^* = &\argmax_{\textbf{Q}} \log\left|\det(\textbf{Q})\right|\\
	    s.t. \quad \matr{Q}\tilde{\textbf{P}} \succeq 0& \quad and \quad \textbf{1}_K^\transpose \matr{Q}\tilde{\textbf{P}}=\textbf{1}_M^\transpose.
	\end{split}
\end{equation}
%
Note that (\ref{eq:eq6}) is non-concave and may have many local maxima which is difficult to find the global optima. Li et al. \cite{li2008minimum} proposed a sequential quadratic programming (SQP) algorithm to find the sub-optimal solutions of (\ref{eq:eq6}) which will be described as follows.

We first simplify the constraint $\textbf{1}_K^\transpose \matr{Q}\tilde{\textbf{P}}=\textbf{1}_M^\transpose$. Note that the every column of $\tilde{\matr{P}}$ can be represented as a linear combination of $K$ linearly independent vectors picked among the columns of $\tilde{\matr{P}}$: let the $K$ linearly independent vectors be expressed as the matrix $\matr{P}_K=[\tilde{\matr{p}}_{i_1} \; \ldots \; \tilde{\matr{p}}_{i_K}]$. Every column of $\tilde{\matr{P}}$ can be written as $\tilde{\matr{p}}=\matr{P}_K \beta$, where $\textbf{1}_K^\transpose\beta=1$. Consequently, we can re-write the constraint as the equality constraint $\textbf{1}_K^\transpose \matr{Q}=\textbf{1}_K^\transpose \matr{P}_K^{-1}\equiv \matr{c}$ where $\matr{c}=\textbf{1}^\transpose\matr{P}_K ^{-1}$ which is a constant row vector. Hence, the problem (\ref{eq:eq6}) becomes:
%
\begin{equation}
	\label{eq:eq7}
	\begin{split}
	    \textbf{Q}^* = &\argmax_{\textbf{Q}} \log\left|\det(\textbf{Q})\right|\\
	    s.t. \quad \matr{Q}\tilde{\textbf{P}} \succeq 0& \quad and \quad \textbf{1}_K^\transpose \matr{Q}=\matr{c}.
	\end{split}
\end{equation}
%

Li et al. \cite{li2008minimum} provided an SQP-based algorithm to solve the problem in (\ref{eq:eq7}). They first applied the output of the Vertex Component Analysis (VCA) algorithm \cite{nascimento2005vertex} for initialization. The output of VCA is a set of $K$ vectors from the columns of $\tilde{\matr{P}}$ the projected utterance points of the given corpus. To lighten the computation, we can discard the points inside the convex hull generated by the $K$ VCA vectors. To further speedup the algorithm, we can expand convex hull so that more points are inside and can thus be discarded. The details of the algorithm for solving Problem (\ref{eq:eq7}) is shown in Algorithm 1.

\begin{algorithm}
\KwInput{ $p,Y, (f(Q)\equiv log|det(Q)|)$ }
\KwOutput{matrix $Q$}
\begin{algorithmic}[1]

\State $Q_o := VCA(Y, 'Endmembers',p) $
\State $Q_o := expand(M)$
\State $Y := discard(Y);$ if y is inside the simplex
\State Inequality constraint

$A * Q \geq b, A = Y^T \otimes I_p, b=0_{pn}$
\State Equality Constraint

$Aeq*Q=beq, Aeq=I_p \otimes I^T_p, beq =q_m^T$\
\State $g(Q) := -(Q^{-1})^T, $ where $g(Q)$ is the gradient of $f$
\State $[H(Q)]_{i,j} := -[g(Q)_{:,j}*g(Q)_{i,:}]$, 

where $H(Q)$ is the Hessian matrix of $f$
\State $Q:=SQP(f, Q_o, A,b, Aeq, beq, g,H)$
\end{algorithmic}
\caption{Minimum Volume Simplex Analysis (MVSA)}
\end{algorithm}

==> proposals and backups/graph_learning_proposal.tex <==
Description: CPM reveals utterance specific word-word relationship related to semantic frames. As a natural extension, we would expect the contextual embeddings of encoded words to reflect such relationship in nn model, and CPM generated word-word coefficients are expected to be helpful in this process. We therefore incorporate concepts in neural graph learning, and add a loss function penalizing encoded features of words distant from that of semantically related words, as determined by coefficient value. The new loss is added with the slot filling loss (with weights applied) to guide the training process.



Work in Progress as of 16/02/2021

18/02 update: performance is fine (pending tuning). Thinking about graph embedding in general

==> proposals and backups/methodology_old.tex <==
\section{Methodology}
Main aim of the work and principal conclusions.

% \section{Rationale of the Convex Polytopic Model}
\textbf{Objective:} Show the interpretability and transparency (and beauty) of our model.
% Enhance the interpretability...

\textbf{Plan:} In this section, we will explain the detailed steps of CPM, along with resulting properties and illustrative examples. We will specify:
\begin{enumerate}
    \item \textcolor{green} {illustrative examples(like those in slides)}
    \item \textcolor{red}{experiments on datasets (write in experiment section}
\end{enumerate}


\subsection{Intuition? Assumption? }
Tokens and their combinations can define the scope of a corpus. \textcolor{red}{[Need support]}
However, a more compact scope of the corpus is defined by the semantic concepts(patterns?) that constituents the utterances in the corpus.
All the utterances within the scope of the corpus can be described as a combination of the semantic patterns. 
Meanwhile, the meaning of an utterance can be constructed by the meaning of its parts. (ref: chapter 18 of SLP, 2nd Eidtion) %connect this to dependency parsing? syntax analysis?

Therefore, we propose this framework, which can:
1. find the semantic patterns in the corpus;
2. discover the relationship between the utterances and the semantic patterns.
This framework is based the convex polytopic model which is used to generate a compact convex polytope to enclose all the data points. The convex polytope defines the scope of the corpus. Also, the semantic patterns can be derived from the extreme points (i.e. vertices) of the polytope.

% Consider

% \textbf{Notes:}
% \begin{enumerate}
%     \item be aware of geometric proprieties and linguistic properties.
%     \item  use a fake dataset for illustration?
% \end{enumerate}
\subsection{detailed structure}
    \\CPM steps:
    \begin{enumerate}
        \item pre-processing utterances (ignore)
        \item   utterances -sum-normalized TDM->points . This step introduces following properties:
        \begin{enumerate}
            
            \item The utterances are first transformed into a sum-normalized TDM and X, where the $X_ij$ is the frequency of the $i-$th term in the $j-$th utterance. And the \textbf{Euclidean distances} between data points measures the distances between them.  (\textcolor{red}{[Experiment 1? : show that the closer the utterance points are, the more similar they are to each other})
            
            \item the utterances that contain fewer semantic patterns tend to be the extreme points (i.e. lie further away from the centre of the hyperplane).  (\textcolor{red}{Experiment 2? : show some furthest utterance points (preliminary result: ``what is aircode?";``"show flights from city name to city name"} )
        \end{enumerate}
        
        \item Embed the utterance points onto a lower dimensional subspace: points -PCA-> a lower-dimensional subspace. [Reason for PCA, not certain] Finding convex polytope on the original high dimension subspace is not a trivial work. Therefore, we aim to find a closest low-dimensional subspace for the utterance points. \textcolor{green}{Example 1: point set}   % what if no PCA? like on a small corpus, directly find convex polytope?
        
        This step introduces following properties:
            \begin{enumerate}
                \item PCA finds the principle components that corresponds to the direction where the data has the largest variance. and we will find the compact convex polytope on this lower-dimensional subspace. 
                \item As PCA preserves the distinctive features of the utterance points, the extreme points remain extreme after PCA projection. Higher dimension preserves more features
                %\item Note that not all the extreme points remains extreme now, as some features are compressed. Therefore, the features founded by CPM is filtered by PCA 
            \end{enumerate}
            %[No Need to mention properties of the principle compoents, as we are not going to use it] \item Question : what are the PCA components? :   are fitted into the R-D ellipsoid, the axes of the ellipsoid are principal components -> data has largest variance along which direction (most distinguishable features) -> \textcolor{red}{Assumption missing here, e.g., on linguistic level, semantic patterns are the features that distinguishes the corpus} ->
        
        \item Generate a compact convex polytope to enclose the embedded utterances
        There are several ways to generate a convex polytope.
        \begin{enumerate}
            \item NO-type [pros: minimal volume]: here we should use example to validate this framework (in the assumption section) \textcolor{green}{Example 2: NO};  \textcolor{red}{Experiment  3: a. Scope? [experiment can be done using DSTC dataset] b. Patterns? }
            \item MVS-type [pros: extract patterns from corpus]:\textcolor{green}{Example 3: 2D MVS} \textcolor{red}{Experiment 4: 2D MVS}  Also, here we should mention how to interpret vertices:
            \begin{enumerate}
            \item directly using coordinates: utterance = composition of semantic concepts embedding (convex representation directly fed to neural network) 
            \item  on the original TDM-spanned space: coordinates -> topwords (related to pattern and chaining) or coordinates -> token importance to vertices (attention) \textcolor{red}{Experiment 5: token representation (attention heat map)}
                \item euclidean distances (k-means) (knn) \textcolor{red}{Experiment 6: pattern formation and comparing to Stanford parser}
         \end{enumerate}
     
            % what does the previously found 2D type polytope looks like on the 3D subspace?}
        \end{enumerate}
    \end{enumerate}

% \subsection{Convex Polytopic Model}
%     In this section, we will explain the detailed steps of CPM, along with resulting properties and illustrative examples. 
%     CPM involves two major steps. First, the utterances are embedded into a low-dimensional affine subspace by Principal Component Analysis (PCA). 
    
%     Second, A convex polytope is subsequently computed, enclosing all embedded utterance points in the subspace. 
    
    
%     a. PCA
%     The utterances are first prepared as a term-document matrix, where (describe tdm). 
%     Given that we need to extract a limited number of latent features, and the vocabulary size of TDM is usually very large, we perform PCA to reduce the dimension of the vector representation of utterances. (why pca)
    % Additionally, due to the potential inequality of word count in different utterances, the subspace vector of PCA can only be compared by cosine similarity, while word count in utterances influence the norm and the euclidean distance between projected points cannot be used. This can be solved by performing sum-normalization across columns of tdm (i.e. individual utterances) to ensure that the tdm is on a sum-to-one hyperplane. (Why sum-normalization)
%     The pca can then be performed by eigenvaue decomposition on the covariance matrix of the sum-normalized tdm.
%     This is in contrast to traditional lsa where no normalization is pre-applied and the result can only be utlized through cosine similarity. The result are utterance points projected to low dimensional space, with the dataset having largest variance along the principle components. (expand a little bit here with the description above)
%     (example: correlation matrix of lsa and pca on the dataset. expect to see that first component of lsa is somewhat related to other components, while not obvious in the pca, which is desired since we are not wasting components)
%     b. NO/MVS
%   While the basis of pca can be interpreted as latent features in the corpus, the coefficients of such features (i.e. coordinates of points) are not bounded in non-negative real number space, which renders the explanation more difficult, since we want to decompose linguistic concepts to utterances, and it is hard to imagine a concept "negatively contributing" to the utterance. We therefore favor a new basis, on top of which all points are the convex combination of the basis vectors. 
   
%   As discussed above, distance between points in the affine subspace is meaningful in describing the similarity between utterances. Following the idea, points at the edge of the utterances set are relatively different to other utterances. If we find the convex set enclosing the utterance points, we can describe any utterance points in the set with at least dimension+1 points in the hull, and to capture the unique concepts, the points should be chosen in the extreme set of such convex hull. To describe the corpus with a set of unique concepts that are still relevant to the utterances, i.e. as close as possible to the utterances points set, we need to find the convex hull of the utt points set. This could be performed using (introduce no and mvs)
%   (explain the difference between no and mvs)
%   (explain mvs algorithm)
% \subsection{Properties}
%     \begin{enumerate}
%         \item utterances are projected to subspace; utterance consisting of concepts of multiple vertices = interior
%         \item vertices capture distinct semantic concepts, which could be derived from the following properties:
%         \begin{enumerate}
%             \item  - projecting back to original tdm-spanned space: coordinates -> topwords (related to pattern and chaining) or coordinates -> token importance to vertices (attention)
%         \item directly using coordinates: utterance = composition of semantic concepts embedding (convex representation directly fed to neural network)
%         \item euclidean distances (k-means) (knn)
%         \end{enumerate}
%     \end{enumerate}


==> proposals and backups/nn_intent_proposal.tex <==
Goal: Further verify that convex coefficient of utterance points that indicating their relationships with the vertices can be used to understand semantic meaning of the utterances; Show that such mechanism is interpretable and transparent in application.

Rationale: 
- Convex coefficients can be used as feature vector of utterances for intent detection
    - Utterances with the same semantic frame shows a high degree of consistency of their radar graph
    - convex coefficients (which is the source of radar graph) should contain information related to semantic frame
    - Intent is an important part of semantic frame
    - Thus, CPM convex coefficients are expected to provide frame knowledge to the intent classification model, such that it could boost performance, and the coefficients are interpretable and transparent, similar arguments as those for slot filling (SF)
- We have investigated CPM and word-level semantic information (SF with CPM attention), however we have not done intent detection (ID), which is often a co-task with many papers training these two tasks jointly
- Heatmap of intents and vertices demonstrated that utterances with the same intents are composed of intent related vertices, so we might want to follow up on it

Added Implementation
- Keep the slot decoder as is
- Additionally, add an intent decoder consisting of a fully-connected layer with softmax activation, with the last decoder state (which should contain the information of the whole input sequence) and the convex coefficient concatenated together as input, and a predicted probability distribution of intent as output
- Use the same loss function of SF on ID. Total loss is calculated with SF loss and ID loss added. The weight of the two sub-task loss should be tuned as a hyperparameter
- Use SF F1 score, ID accuracy (\% of correctly detected intent) and total frame accuracy (\% of utterances with slot and intent completely correctly predicted) as metrics

Baseline: Weighted sum of decoder output at different timesteps as utterance feature vector. The weight is learnt through an additional layer of feed-forward network
(should we add more baselines? this is only an extension to the slot filling only experiment)

Weakness in proof:
- Encoder, slot decoder and intent decoder are jointly trained, the effect of individual knowledge sources, i.e. CPM-generated attention and convex combination coefficients, is not clear
    Partial solution: do three experiments: SF only without intent decoder (already written in the draft), joint SF-ID with different utterance feature vectors for ID (same attention mechanism in SF) (not done yet), joint SF-ID with CPM attention + CPM combination coefficients compared to feed-forward attention + feed forward coefficients (in progress, preliminary results are solid)
    First experiment: CPM attention works; Second experiment: CPM combination coefficient works; Third experiment: adding them together for a showcase in actual SF-ID performance, demonstrating potential in real application
- The combination coefficients are less interpretable than attention. e.g. what does each dimension in the feature vector refer to?
    Explanation: vertices are related to semantic patterns (in experiment 1.1.1), are related to intents (in experiment 1.1.2), thus they refer to semantic concepts related to semantic frames. Thus, each utterance could be viewed as a combination of such semantic concepts.

==> punctuation.tex <==
concepts:
new concepts(semantic patterns, etc.): italics
emphasize existing points: bold

intents:
uppercase

slots:
small caps

categories(city_name, etc.):
italics

math variables:
scalar: italics
vector/matrix: mathbf(~bold)

==> tables/ff_schema.tex <==
\begin{figure}
\begin{minipage}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/ff_18.png}
    \caption{uni-sechma-1}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/ff_65.png}
    \caption{uni-sechma-2}
    \label{fig:uni-sechma}
    \end{minipage}
\end{figure}

==> tables/graph.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c | c | c | c|}
\hline
%  \toprule
    \multicolumn{4}{c|}{Data size}\\
    \hline
     2.5\% & 5\% & 10\% & 90\% \\
     \hline
 %  \midrule
    61.2/75.81/25.53 & 75.07/78.84/40.87 & 83.16/83.99/55.77 & 94.76/95.19/83.09\\
    \hline
%\bottomrule
\end{tabular}
\caption{Result of CPM vertex-base neural graph learning on different annotated training data size (in percentage of 4978 training utterances), reported in the format of slot filling F1 score/intent classification accuracy(\%)/frame accuracy(\%)}
\label{tab:graph}
\end{table}

==> tables/intent.tex <==
\begin{table}[h]
\centering
\begin{tabular}{c  c  c  c  c  c}
%  \toprule
\hline
    \multirow{2}{*}{Feature vector source} & \multicolumn{4}{c}{Data size}\\
    \cline{2-5}
    & 2.5\% & 5\% & 10\% & 90\% \\
 %  \midrule
 \hline
    All-ones vector & 81.99 & 81.97 & 84.77 & 94.18 \\
    \hline
    CPM & \textbf{82.46} & \textbf{84.43} & \textbf{85.33} & \textbf{95.97} \\
    \hline
%bottomrule
\end{tabular}
\caption{Accuracy(\%) of predicted intent labels on different training data size (in percentage of 4978 training utterances) and different feature vector sources. Feature vector generated using CPM achieve better intent classification accuracy on all sizes of training dataset.}
\label{tab:intent}
\end{table}

==> tables/joint.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c  c  c  c  c|}
%  \toprule
\hline
\multirow{2}{*}{Model}& \multicolumn{4}{c|}{Data size}\\
\cline{2-5}
      & 2.5\% & 5\% & 10\% & 90\% \\
 %  \midrule
 \hline
     Baseline & 55.16/68.31/21.28 & 71.61/83.76/39.31	& 81.80/85.67/54.31 & 94.34/96.75/\textbf{83.87} \\
    \hline
    CPM & 54.60/78.39/\textbf{23.40} & 76.21/83.87/\textbf{43.56} & 83.48/89.25/\textbf{58.23} & 94.46/96.75/83.54 \\
    \hline

%\bottomrule
\end{tabular}
\caption{Result of joint learning on different training data size (in percentage of 4978 training utterances), reported in the format of slot filling F1 score/intent classification accuracy(\%)/frame accuracy(\%)}
\label{tab:joint}
\end{table}

==> tables/radar.tex <==

\begin{figure}
    \centering
    \subfloat[Radar graph of five utterances with the same semantic frame. ]{
    \includegraphics[width=0.45\linewidth,valign=B]{figs/radar_frame_1.png}}
       \quad
   \subfloat[Five utterances with the same semantic frame and four most important vertices.]{\includegraphics[width=0.45\linewidth,valign=B]{figs/radar-table-1.png}} 
    \\
    \caption{Compositional analyze result of five utterances with the same semantic frame}
    \label{fig:radar-1}
\end{figure}


\begin{figure}
    \centering
    \subfloat[Radar graph of five randomly selected utterances. ]{
    \includegraphics[width=0.45\linewidth,valign=B]{figs/radar_rand_1.png}}
    \quad
   \subfloat[Five randomly selected utterances and four most important vertices。]{\includegraphics[width=0.45\linewidth,valign=B]{figs/radar-table-2.png}} 
    \\
    \caption{Compositional analyze result of five randomly selected utterances}
    \label{fig:radar-2}
\end{figure}



==> tables/schamaball-old.tex <==

\begin{figure}
    \centering
    \subfloat[ `all flights from denver to pittsburgh leaving after 6 pm and before 7 pm' (no contextual information)]{
    \includegraphics[width=0.45\linewidth,valign=B]{figs/pure_18.png}}
   \quad
   \subfloat[`which airlines have first class flights today' (no contextual information)]{\includegraphics[width=0.45\linewidth,valign=B]{figs/pure_65.png}} 
    \\
    \subfloat[`all flights from denver to pittsburgh leaving after 6 pm and before 7 pm' (with contextual information)]{
    \includegraphics[width=0.45\linewidth,valign=B]{figs/weighted_18.png}}
    \quad
   \subfloat[ `which airlines have first class flights today' (with contextual information)]{\includegraphics[width=0.45\linewidth,valign=B]{figs/weighted_65.png}} 
   \\
    \caption{Schema-balls of word-word correlation in the utterances (a, b: no contextual information; c, d: with contextual information). Nodes are words in the utterance and are arranged anti-clockwise. The thickness of the line between two nodes indicates the correlation strength between two words from the perspective of semantic patterns.}
    \label{fig:uni-sechma}
\end{figure}

